Faster and shorter synthesis of Hamiltonian simulation circuits

We devise greedy heuristics tailored for synthesizing quantum circuits that implement a specified set of Pauli rotations. Our heuristics are designed to minimize either the count of entangling gates or the depth of entangling gates, and they can be adjusted to either maintain or loosen the ordering of rotations. We present benchmark results demonstrating a depth reduction of up to a factor of 4 compared to the current state-of-the-art heuristics for synthesizing Hamiltonian simulation circuits. We also show that these heuristics can be used to optimize generic quantum circuits by decomposing and resynthesizing them.

==> table.tex <==

\begin{table}
\centering
\scalebox{0.8}{
\hspace*{-4.5cm}\begin{tabular}{|c|cc|cccc|cccc|}
     \hline
    ~   & \multicolumn{2}{c|}{Duncan et al.} & \multicolumn{4}{c|}{Greedy count} & \multicolumn{4}{c|}{Greedy depth} \\
     mol./orbitals/enc./basis  & count & depth & count & rel. count & depth & rel. depth & count & rel. count & depth & rel. depth\\
        \hline
H2/cmplt/BK/sto3g & 14 & 14 & 9 & -35.71\% &9 & -35.71\% &11 & -21.43\% &6 & -57.14\% \\
H2/cmplt/P/sto3g & 14 & 14 & 10 & -28.57\% &9 & -35.71\% &18 & 28.57\% &10 & -28.57\% \\
H2/cmplt/JW/sto3g & 22 & 18 & 11 & -50.00\% &7 & -61.11\% &21 & -4.55\% &11 & -38.89\% \\
H2/cmplt/JW/631g & 222 & 181 & 117 & -47.30\% &87 & -51.93\% &182 & -18.02\% &58 & -67.96\% \\
H2/cmplt/BK/631g & 236 & 228 & 109 & -53.81\% &82 & -64.04\% &215 & -8.90\% &69 & -69.74\% \\
H2/cmplt/P/631g & 271 & 262 & 115 & -57.56\% &87 & -66.79\% &201 & -25.83\% &66 & -74.81\% \\
H4/cmplt/BK/sto3g & 338 & 293 & 233 & -31.07\% &175 & -40.27\% &378 & 11.83\% &120 & -59.04\% \\
H4/cmplt/JW/sto3g & 385 & 302 & 213 & -44.68\% &141 & -53.31\% &363 & -5.71\% &111 & -63.25\% \\
LiH/frz/JW/sto3g & 430 & 344 & 184 & -57.21\% &132 & -61.63\% &448 & 4.19\% &114 & -66.86\% \\
H4/cmplt/P/sto3g & 457 & 377 & 258 & -43.54\% &182 & -51.72\% &351 & -23.19\% &108 & -71.35\% \\
LiH/frz/P/sto3g & 527 & 499 & 228 & -56.74\% &154 & -69.14\% &396 & -24.86\% &102 & -79.56\% \\
LiH/frz/BK/sto3g & 573 & 491 & 233 & -59.34\% &190 & -61.30\% &455 & -20.59\% &115 & -76.58\% \\
NH/frz/JW/sto3g & 962 & 771 & 678 & -29.52\% &477 & -38.13\% &1142 & 18.71\% &284 & -63.16\% \\
NH/frz/P/sto3g & 1411 & 1152 & 649 & -54.00\% &475 & -58.77\% &1133 & -19.70\% &279 & -75.78\% \\
NH/frz/BK/sto3g & 1623 & 1350 & 623 & -61.61\% &440 & -67.41\% &1001 & -38.32\% &251 & -81.41\% \\
H2O/frz/JW/sto3g & 1701 & 1338 & 1620 & -4.76\% &1136 & -15.10\% &2325 & 36.68\% &484 & -63.83\% \\
NH/cmplt/JW/sto3g & 1701 & 1338 & 1620 & -4.76\% &1136 & -15.10\% &2325 & 36.68\% &484 & -63.83\% \\
LiH/cmplt/JW/sto3g & 1763 & 1373 & 1651 & -6.35\% &1153 & -16.02\% &2556 & 44.98\% &520 & -62.13\% \\
LiH/cmplt/P/sto3g & 2269 & 1872 & 1613 & -28.91\% &1096 & -41.45\% &2518 & 10.97\% &518 & -72.33\% \\
CH2/frz/JW/sto3g & 2362 & 1786 & 1934 & -18.12\% &1348 & -24.52\% &2971 & 25.78\% &607 & -66.01\% \\
H2O/frz/P/sto3g & 2416 & 1992 & 1476 & -38.91\% &1024 & -48.59\% &2356 & -2.48\% &487 & -75.55\% \\
NH/cmplt/P/sto3g & 2416 & 1992 & 1476 & -38.91\% &1024 & -48.59\% &2356 & -2.48\% &487 & -75.55\% \\
H2/cmplt/JW/ccpvdz & 2880 & 2361 & 904 & -68.61\% &551 & -76.66\% &3136 & 8.89\% &383 & -83.78\% \\
LiH/frz/JW/631g & 2880 & 2361 & 904 & -68.61\% &551 & -76.66\% &3136 & 8.89\% &383 & -83.78\% \\
     \hline
 \end{tabular}}
 \end{table}

\begin{table}
\centering
\scalebox{0.8}{
\hspace*{-4.5cm}\begin{tabular}{|c|cc|cccc|cccc|}
     \hline
    ~   & \multicolumn{2}{c|}{Duncan et al.} & \multicolumn{4}{c|}{Greedy count} & \multicolumn{4}{c|}{Greedy depth} \\
     mol./orbitals/enc./basis  & count & depth & count & rel. count & depth & rel. depth & count & rel. count & depth & rel. depth\\
        \hline
H2O/frz/BK/sto3g & 2965 & 2343 & 1478 & -50.15\% &1009 & -56.94\% &2427 & -18.15\% &503 & -78.53\% \\
NH/cmplt/BK/sto3g & 2965 & 2343 & 1478 & -50.15\% &1009 & -56.94\% &2427 & -18.15\% &503 & -78.53\% \\
LiH/cmplt/BK/sto3g & 3059 & 2397 & 1440 & -52.93\% &991 & -58.66\% &2342 & -23.44\% &490 & -79.56\% \\
H2/cmplt/BK/ccpvdz & 3072 & 2664 & 759 & -75.29\% &473 & -82.24\% &3316 & 7.94\% &408 & -84.68\% \\
LiH/frz/BK/631g & 3072 & 2664 & 759 & -75.29\% &473 & -82.24\% &3316 & 7.94\% &408 & -84.68\% \\
H2O/cmplt/JW/sto3g & 3074 & 2431 & 2863 & -6.86\% &1957 & -19.50\% &3943 & 28.27\% &692 & -71.53\% \\
CH2/frz/P/sto3g & 3454 & 2658 & 1975 & -42.82\% &1312 & -50.64\% &3221 & -6.75\% &652 & -75.47\% \\
H2/cmplt/P/ccpvdz & 3454 & 3299 & 786 & -77.24\% &469 & -85.78\% &3094 & -10.42\% &386 & -88.30\% \\
LiH/frz/P/631g & 3454 & 3299 & 786 & -77.24\% &469 & -85.78\% &3094 & -10.42\% &386 & -88.30\% \\
CH2/frz/BK/sto3g & 4047 & 3042 & 1974 & -51.22\% &1351 & -55.59\% &3055 & -24.51\% &620 & -79.62\% \\
CH2/cmplt/JW/sto3g & 4349 & 3510 & 4260 & -2.05\% &2812 & -19.89\% &6523 & 49.99\% &1123 & -68.01\% \\
H4/cmplt/JW/631g & 4506 & 3570 & 4921 & 9.21\% &3168 & -11.26\% &6352 & 40.97\% &969 & -72.86\% \\
H2O/cmplt/P/sto3g & 4546 & 3704 & 3134 & -31.06\% &2122 & -42.71\% &4461 & -1.87\% &788 & -78.73\% \\
H2O/cmplt/BK/sto3g & 4851 & 3800 & 2771 & -42.88\% &1835 & -51.71\% &4105 & -15.38\% &725 & -80.92\% \\
H4/cmplt/BK/631g & 5518 & 4358 & 3770 & -31.68\% &2464 & -43.46\% &7570 & 37.19\% &1131 & -74.05\% \\
H4/cmplt/P/631g & 5738 & 4691 & 3266 & -43.08\% &2126 & -54.68\% &7511 & 30.90\% &1141 & -75.68\% \\
CH2/cmplt/P/sto3g & 6247 & 4887 & 4255 & -31.89\% &2699 & -44.77\% &6458 & 3.38\% &1115 & -77.18\% \\
CH2/cmplt/BK/sto3g & 7754 & 5590 & 3864 & -50.17\% &2452 & -56.14\% &6663 & -14.07\% &1150 & -79.43\% \\
H8/cmplt/JW/sto3g & 7806 & 6215 & 8816 & 12.94\% &5603 & -9.85\% &13904 & 78.12\% &2057 & -66.90\% \\
H8/cmplt/BK/sto3g & 9275 & 7095 & 8767 & -5.48\% &5565 & -21.56\% &13647 & 47.14\% &2017 & -71.57\% \\
H8/cmplt/P/sto3g & 10077 & 7779 & 8596 & -14.70\% &5461 & -29.80\% &13447 & 33.44\% &1983 & -74.51\% \\
LiH/frz/BK/ccpvdz & 11490 & 9978 & 2682 & -76.66\% &1635 & -83.61\% &24804 & 115.87\% &1580 & -84.17\% \\
LiH/cmplt/JW/631g & 12316 & 10071 & 5404 & -56.12\% &3323 & -67.00\% &21609 & 75.45\% &2331 & -76.85\% \\
LiH/frz/JW/ccpvdz & 14708 & 12885 & 2815 & -80.86\% &1672 & -87.02\% &24353 & 65.58\% &1553 & -87.95\% \\
LiH/frz/P/ccpvdz & 16730 & 16312 & 2904 & -82.64\% &1574 & -90.35\% &23179 & 38.55\% &1488 & -90.88\% \\
     \hline
 \end{tabular}}
 \end{table}

\begin{table}
\centering
\scalebox{0.8}{
\hspace*{-4.5cm}\begin{tabular}{|c|cc|cccc|cccc|}
     \hline
    ~   & \multicolumn{2}{c|}{Duncan et al.} & \multicolumn{4}{c|}{Greedy count} & \multicolumn{4}{c|}{Greedy depth} \\
     mol./orbitals/enc./basis  & count & depth & count & rel. count & depth & rel. depth & count & rel. count & depth & rel. depth\\
        \hline
LiH/cmplt/P/631g & 17866 & 14372 & 5582 & -68.76\% &3368 & -76.57\% &20217 & 13.16\% &2187 & -84.78\% \\
NH/frz/JW/631g & 18047 & 14285 & 20787 & 15.18\% &12509 & -12.43\% &31046 & 72.03\% &3626 & -74.62\% \\
NH/frz/P/631g & 21655 & 16275 & 21164 & -2.27\% &12827 & -21.19\% &30731 & 41.91\% &3590 & -77.94\% \\
LiH/cmplt/BK/631g & 22504 & 16252 & 6453 & -71.33\% &3909 & -75.95\% &18608 & -17.31\% &2015 & -87.60\% \\
NH/frz/BK/631g & 27732 & 19801 & 20478 & -26.16\% &12396 & -37.40\% &31339 & 13.01\% &3673 & -81.45\% \\
NH/cmplt/JW/631g & 32151 & 24822 & 40919 & 27.27\% &24074 & -3.01\% &64547 & 100.76\% &6740 & -72.85\% \\
H2/cmplt/BK/ccpvtz & 34574 & 30481 & 6650 & -80.77\% &4213 & -86.18\% &102786 & 197.29\% &4118 & -86.49\% \\
NH/cmplt/P/631g & 37051 & 27392 & 42617 & 15.02\% &25058 & -8.52\% &63433 & 71.20\% &6648 & -75.73\% \\
H2O/frz/JW/631g & 37964 & 29856 & 62307 & 64.12\% &35503 & 18.91\% &92708 & 144.20\% &8827 & -70.43\% \\
H2O/frz/BK/631g & 45407 & 33333 & 56338 & 24.07\% &32358 & -2.93\% &91185 & 100.82\% &8723 & -73.83\% \\
H2O/frz/P/631g & 45898 & 34351 & 58916 & 28.36\% &33172 & -3.43\% &93256 & 103.18\% &8850 & -74.24\% \\
NH/cmplt/BK/631g & 47440 & 33883 & 40039 & -15.60\% &23336 & -31.13\% &65782 & 38.66\% &6877 & -79.70\% \\
H2/cmplt/JW/ccpvtz & 51498 & 46965 & 7033 & -86.34\% &3859 & -91.78\% &101498 & 97.09\% &4058 & -91.36\% \\
C2H4/frz/JW/sto3g & 51714 & 39273 & 74775 & 44.59\% &42990 & 9.46\% &126041 & 143.73\% &11866 & -69.79\% \\
H2/cmplt/P/ccpvtz & 56526 & 55687 & 6396 & -88.68\% &3960 & -92.89\% &105599 & 86.81\% &4214 & -92.43\% \\
LiH/cmplt/JW/ccpvdz & 65384 & 56290 & 21405 & -67.26\% &11094 & -80.29\% &133170 & 103.67\% &7911 & -85.95\% \\
H2O/cmplt/JW/631g & 65909 & 50811 & 100335 & 52.23\% &55689 & 9.60\% &167906 & 154.75\% &14569 & -71.33\% \\
C2H4/frz/P/sto3g & 68723 & 48918 & 75678 & 10.12\% &43338 & -11.41\% &119648 & 74.10\% &11279 & -76.94\% \\
H4/cmplt/BK/ccpvdz & 71068 & 56262 & 21008 & -70.44\% &11531 & -79.50\% &162492 & 128.64\% &9153 & -83.73\% \\
H4/cmplt/JW/ccpvdz & 73526 & 63700 & 17300 & -76.47\% &9625 & -84.89\% &161463 & 119.60\% &9165 & -85.61\% \\
LiH/cmplt/BK/ccpvdz & 78685 & 59653 & 15774 & -79.95\% &9241 & -84.51\% &137211 & 74.38\% &8167 & -86.31\% \\
LiH/cmplt/P/ccpvdz & 83843 & 67600 & 16612 & -80.19\% &9329 & -86.20\% &137173 & 63.61\% &8198 & -87.87\% \\
H4/cmplt/P/ccpvdz & 88082 & 71296 & 19720 & -77.61\% &10257 & -85.61\% &161833 & 83.73\% &9140 & -87.18\% \\
H2O/cmplt/P/631g & 92077 & 65966 & 106377 & 15.53\% &59082 & -10.44\% &166504 & 80.83\% &14455 & -78.09\% \\
C2H4/frz/BK/sto3g & 94650 & 61735 & 76145 & -19.55\% &43922 & -28.85\% &124396 & 31.43\% &11733 & -80.99\% \\
     \hline
 \end{tabular}}
 \end{table}

\begin{table}
\centering
\scalebox{0.8}{
\hspace*{-4.5cm}\begin{tabular}{|c|cc|cccc|cccc|}
     \hline
    ~   & \multicolumn{2}{c|}{Duncan et al.} & \multicolumn{4}{c|}{Greedy count} & \multicolumn{4}{c|}{Greedy depth} \\
     mol./orbitals/enc./basis  & count & depth & count & rel. count & depth & rel. depth & count & rel. count & depth & rel. depth\\
        \hline
C2H4/cmplt/JW/sto3g & 102575 & 78029 & 165582 & 61.43\% &89802 & 15.09\% &266020 & 159.34\% &21262 & -72.75\% \\
C2H4/cmplt/P/sto3g & 121559 & 87877 & 165085 & 35.81\% &89813 & 2.20\% &282875 & 132.71\% &22527 & -74.37\% \\
H2O/cmplt/BK/631g & 127118 & 79942 & 105657 & -16.88\% &59030 & -26.16\% &171161 & 34.65\% &14849 & -81.43\% \\
C2H4/cmplt/BK/sto3g & 177411 & 113172 & 155795 & -12.18\% &82544 & -27.06\% &262623 & 48.03\% &21009 & -81.44\% \\
     \hline
 \end{tabular}}
 \end{table}


==> table_new.tex <==

\begin{table}[]
    \centering

\begin{tabular}{lrrrrr}
\toprule
 & naive & ph & tket & rdepth & rcount \\
 & count & count & count & count & count \\
name &  &  &  &  &  \\
\midrule
LiH cmplt JW sto3g & 38 & -31.5\% & -52.6\% & -68.4\% & {\cellcolor{green}} -71.0\% \\
LiH frz P sto3g & 38 & -31.5\% & -57.8\% & -71.0\% & {\cellcolor{green}} -73.6\% \\
H2O cmplt P sto3g & 56 & -28.5\% & -60.7\% & {\cellcolor{green}} -78.5\% & {\cellcolor{green}} -78.5\% \\
C2H4 cmplt JW sto3g & 630 & -54.7\% & -67.6\% & {\cellcolor{green}} -82.6\% & -81.4\% \\
H2 cmplt P ccpvdz & 666 & -53.1\% & -62.0\% & -78.3\% & {\cellcolor{green}} -79.8\% \\
LiH cmplt BK ccpvdz & 768 & -61.8\% & -73.8\% & -82.1\% & {\cellcolor{green}} -82.9\% \\
H2 cmplt JW ccpvdz & 1448 & -61.8\% & -66.5\% & {\cellcolor{green}} -83.0\% & -80.7\% \\
H2O cmplt JW 631g & 1316 & -53.4\% & -64.5\% & -79.4\% & {\cellcolor{green}} -80.9\% \\
C2H4 frz JW sto3g & 1440 & -56.6\% & -71.4\% & -79.7\% & {\cellcolor{green}} -81.5\% \\
H2O cmplt P 631g & 1442 & -64.0\% & -69.6\% & {\cellcolor{green}} -85.7\% & -82.3\% \\
H2O frz BK 631g & 1616 & -69.3\% & -76.3\% & -83.7\% & {\cellcolor{green}} -84.9\% \\
NH frz P sto3g & 1316 & -59.8\% & -65.9\% & -76.5\% & {\cellcolor{green}} -81.4\% \\
H4 cmplt JW ccpvdz & 3700 & -59.6\% & -64.8\% & -76.4\% & {\cellcolor{green}} -79.2\% \\
LiH cmplt BK 631g & 3896 & -63.0\% & -75.7\% & -77.0\% & {\cellcolor{green}} -79.4\% \\
H4 cmplt BK ccpvdz & 4178 & -67.4\% & -71.3\% & {\cellcolor{green}} -81.7\% & -79.7\% \\
H2 cmplt JW 631g & 7640 & -65.4\% & -72.1\% & -72.9\% & {\cellcolor{green}} -75.5\% \\
LiH frz JW ccpvdz & 8064 & -67.8\% & {\cellcolor{green}} -78.6\% & -75.2\% & -77.2\% \\
LiH cmplt BK sto3g & 8064 & -67.8\% & {\cellcolor{green}} -78.6\% & -75.2\% & -77.2\% \\
LiH cmplt JW 631g & 8064 & -72.0\% & -78.6\% & -72.3\% & {\cellcolor{green}} -79.0\% \\
NH cmplt P sto3g & 7796 & -64.1\% & -70.2\% & -74.0\% & {\cellcolor{green}} -75.7\% \\
LiH frz BK sto3g & 7796 & -64.1\% & -70.2\% & -74.0\% & {\cellcolor{green}} -75.7\% \\
NH frz P 631g & 8004 & -68.2\% & -73.4\% & -73.5\% & {\cellcolor{green}} -78.6\% \\
CH2 cmplt P sto3g & 8004 & -68.2\% & -73.4\% & -73.5\% & {\cellcolor{green}} -78.6\% \\
H8 cmplt JW sto3g & 8680 & -75.2\% & -75.8\% & -74.7\% & {\cellcolor{green}} -78.9\% \\
H2 cmplt P ccpvtz & 11344 & -78.5\% & -77.6\% & -84.0\% & {\cellcolor{green}} -85.0\% \\
\bottomrule
\end{tabular}
    
    \caption{Entangling count comparison for UCCSD Ansätze synthesis for different molecules, encodings, and bases. The first column displays the naive entangling gate count obtained by individually synthesizing each rotation using two CNOT ladders. Other columns display the entangling gate count gain with respect to that value. The best result of each row is outlined in green.}
    \label{tab:tab_chem_1}
\end{table}
\begin{table}
\begin{tabular}{lrrrrr}
\toprule
 & naive & ph & tket & rdepth & rcount \\
 & count & count & count & count & count \\
name &  &  &  &  &  \\
\midrule
H2 cmplt P ccpvtz & 11344 & -78.5\% & -77.6\% & -84.0\% & {\cellcolor{green}} -85.0\% \\
H2O frz JW sto3g & 11344 & -78.5\% & -77.6\% & -84.0\% & {\cellcolor{green}} -85.0\% \\
C2H4 frz BK sto3g & 10344 & -70.0\% & -76.2\% & -73.7\% & {\cellcolor{green}} -78.3\% \\
H4 cmplt BK sto3g & 9938 & -64.8\% & -67.5\% & -72.3\% & {\cellcolor{green}} -75.8\% \\
H2 cmplt BK ccpvdz & 13878 & -79.9\% & -76.4\% & -88.4\% & {\cellcolor{green}} -90.5\% \\
H2 cmplt P sto3g & 13878 & -79.9\% & -76.4\% & -88.4\% & {\cellcolor{green}} -90.5\% \\
H2O cmplt JW sto3g & 10228 & -70.8\% & -68.2\% & -72.5\% & {\cellcolor{green}} -76.9\% \\
LiH cmplt P ccpvdz & 14616 & -84.3\% & -81.6\% & -87.0\% & {\cellcolor{green}} -89.3\% \\
LiH frz BK 631g & 14616 & -84.3\% & -81.6\% & -87.0\% & {\cellcolor{green}} -89.3\% \\
H2O frz BK sto3g & 13108 & -70.4\% & -73.6\% & {\cellcolor{green}} -74.1\% & -73.1\% \\
LiH frz JW sto3g & 14360 & -68.6\% & -79.9\% & -69.9\% & {\cellcolor{green}} -81.2\% \\
C2H4 cmplt P sto3g & 14020 & -67.9\% & -70.5\% & -72.2\% & {\cellcolor{green}} -76.1\% \\
LiH frz BK ccpvdz & 17924 & -69.7\% & {\cellcolor{green}} -74.3\% & -57.6\% & -69.7\% \\
LiH cmplt P 631g & 21072 & -72.1\% & {\cellcolor{green}} -78.9\% & -70.2\% & -76.2\% \\
H4 cmplt BK 631g & 19574 & -69.1\% & -69.2\% & -67.7\% & {\cellcolor{green}} -73.8\% \\
H8 cmplt BK sto3g & 20514 & -67.8\% & -68.0\% & -68.2\% & {\cellcolor{green}} -74.7\% \\
NH frz JW 631g & 22316 & -72.4\% & {\cellcolor{green}} -76.1\% & -76.0\% & -75.5\% \\
CH2 cmplt JW sto3g & 23200 & -79 & -81.9\% & -68.7\% & {\cellcolor{green}} -82.5\% \\
CH2 cmplt BK sto3g & 37272 & {\cellcolor{green}} -74.9\% & -74.1\% & -60.3\% & -70.8\% \\
C2H4 frz P sto3g & 42368 & -75.2\% & {\cellcolor{green}} -80.5\% & -66.3\% & -75.9\% \\
H4 cmplt P sto3g & 41432 & -70.8\% & -69.6\% & -64.8\% & {\cellcolor{green}} -75.0\% \\
CH2 frz JW sto3g & 49880 & -83.4\% & -79.5\% & -64.7\% & {\cellcolor{green}} -89.2\% \\
H2 cmplt BK ccpvtz & 86598 & -88.5\% & -81.1\% & -82.2\% & {\cellcolor{green}} -93.8\% \\
H4 cmplt P ccpvdz & 89080 & -91.1\% & -84.1\% & -86.1\% & {\cellcolor{green}} -94.1\% \\
H2 cmplt BK sto3g & 53450 & {\cellcolor{green}} -77.6\% & -76.0\% & -76.0\% & -72.1\% \\
\bottomrule
\end{tabular} 
\caption{See table \ref{tab:tab_chem_1} for details}
    \label{tab:tab_chem_2}
\end{table}

\begin{table}

\begin{tabular}{lrrrrr}
\toprule
 & naive & ph & tket & rdepth & rcount \\
 & count & count & count & count & count \\
name &  &  &  &  &  \\
\midrule
H2 cmplt BK sto3g & 53450 & {\cellcolor{green}} -77.6\% & -76.0\% & -76.0\% & -72.1\% \\
H2O cmplt BK sto3g & 67270 & -79.1\% & -79.0\% & -82.0\% & {\cellcolor{green}} -83.9\% \\
H4 cmplt JW sto3g & 69144 & {\cellcolor{green}} -84.5\% & -83.4\% & -78.6\% & -81.6\% \\
H2O cmplt BK 631g & 86650 & {\cellcolor{green}} -76.0\% & -75.0\% & -56.1\% & -74.9\% \\
LiH frz P 631g & 88536 & -80.7\% & {\cellcolor{green}} -82.2\% & -52.6\% & -75.0\% \\
NH cmplt BK 631g & 75664 & {\cellcolor{green}} -77.4\% & -72.3\% & -51.0\% & -69.5\% \\
H2O frz JW 631g & 168986 & -88.8\% & -81.6\% & -49.6\% & {\cellcolor{green}} -91.2\% \\
H2 cmplt BK 631g & 173264 & -81.0\% & {\cellcolor{green}} -82.7\% & -53.2\% & -75.6\% \\
NH cmplt JW 631g & 170666 & {\cellcolor{green}} -77.0\% & -74.6\% & -48.1\% & -73.4\% \\
LiH cmplt P sto3g & 149540 & {\cellcolor{green}} -78.9\% & -73.8\% & -43.0\% & -69.8\% \\
LiH frz P ccpvdz & 335178 & {\cellcolor{green}} -92.5\% & -83.3\% & -75.5\% & -91.7\% \\
CH2 frz BK sto3g & 341280 & -94.2\% & -85.3\% & -79.7\% & {\cellcolor{green}} -95.1\% \\
H4 cmplt JW 631g & 216216 & {\cellcolor{green}} -82.6\% & -80.9\% & -39.6\% & -71.5\% \\
H2O frz P 631g & 241664 & -78.7\% & {\cellcolor{green}} -78.7\% & -48.3\% & -73.4\% \\
LiH cmplt JW ccpvdz & 244992 & -82.2\% & {\cellcolor{green}} -85.7\% & -43.9\% & -78.3\% \\
C2H4 cmplt BK sto3g & 230810 & {\cellcolor{green}} -81.6\% & -78.5\% & -55.1\% & -76.6\% \\
H4 cmplt P 631g & 276768 & {\cellcolor{green}} -83.8\% & -81.8\% & -51.6\% & -79.7\% \\
H8 cmplt P sto3g & 401046 & {\cellcolor{green}} -87.2\% & -84.4\% & -79.3\% & -86.3\% \\
NH cmplt JW sto3g & 407320 & {\cellcolor{green}} -90.9\% & -87.0\% & -74.6\% & -86.3\% \\
NH frz BK sto3g & 312096 & -81.1\% & {\cellcolor{green}} -82.1\% & -52.4\% & -75.0\% \\
NH frz BK 631g & 309068 & {\cellcolor{green}} -77.8\% & -71.5\% & -48.4\% & -73.7\% \\
H2O frz P sto3g & 260656 & {\cellcolor{green}} -79.5\% & -70.6\% & -37.5\% & -69.8\% \\
NH frz JW sto3g & 472132 & {\cellcolor{green}} -87.7\% & -85.3\% & -76.8\% & -85.6\% \\
LiH frz JW 631g & 479136 & {\cellcolor{green}} -91.3\% & -88.2\% & -73.7\% & -85.4\% \\
H2 cmplt JW sto3g & 317504 & {\cellcolor{green}} -78.2\% & -67.4\% & -25.4\% & -65.7\% \\
NH cmplt P 631g & 410000 & {\cellcolor{green}} -79.4\% & -75.1\% & -42.6\% & -72.6\% \\
CH2 frz P sto3g & 414240 & -82.6\% & {\cellcolor{green}} -84.4\% & -44.2\% & -74.8\% \\
NH cmplt BK sto3g & 488548 & {\cellcolor{green}} -78.0\% & -73.7\% & -17.7\% & -65.1\% \\
H2 cmplt JW ccpvtz & 640768 & -82.6\% & {\cellcolor{green}} -86.3\% & -39.0\% & -73.0\% \\
H2 cmplt P 631g & 636668 & {\cellcolor{green}} -80.0\% & -75.5\% & -39.5\% & -73.7\% \\
\bottomrule
\end{tabular}
\caption{See table \ref{tab:tab_chem_1} for details}
    \label{tab:tab_chem_3}
\end{table}
\begin{table}
\begin{tabular}{lrrrrr}
\toprule
 & naive & ph & tket & rdepth & rcount \\
 & depth & depth & depth & depth & depth \\
name &  &  &  &  &  \\
\midrule
LiH cmplt JW sto3g & 32 & -25 & -46.8\% & {\cellcolor{green}} -68.7\% & {\cellcolor{green}} -68.7\% \\
LiH frz P sto3g & 34 & -29.4\% & -58.8\% & -67.6\% & {\cellcolor{green}} -70.5\% \\
H2O cmplt P sto3g & 36 & 5.5\% & -50 & {\cellcolor{green}} -72.2\% & {\cellcolor{green}} -72.2\% \\
C2H4 cmplt JW sto3g & 405 & -33.3\% & -53.8\% & {\cellcolor{green}} -85.6\% & -82.9\% \\
H2 cmplt P ccpvdz & 412 & -26.6\% & -43.2\% & {\cellcolor{green}} -84.9\% & -80.5\% \\
LiH cmplt BK ccpvdz & 436 & -36.9\% & -58.0\% & {\cellcolor{green}} -85.7\% & -79.3\% \\
H2 cmplt JW ccpvdz & 790 & -32.0\% & -42.6\% & {\cellcolor{green}} -87.8\% & -80.1\% \\
H2O cmplt JW 631g & 800 & -29.2\% & -50 & {\cellcolor{green}} -86.1\% & -80.6\% \\
C2H4 frz JW sto3g & 812 & -31.1\% & -60.4\% & {\cellcolor{green}} -85.8\% & -80.4\% \\
H2O cmplt P 631g & 812 & -37.9\% & -48.1\% & {\cellcolor{green}} -90.7\% & -81.2\% \\
H2O frz BK 631g & 832 & -44.2\% & -57.4\% & {\cellcolor{green}} -88.7\% & -81.7\% \\
NH frz P sto3g & 838 & -40.6\% & -53.4\% & {\cellcolor{green}} -86.2\% & -84.0\% \\
H4 cmplt JW ccpvdz & 1947 & -31.0\% & -43.4\% & {\cellcolor{green}} -86.1\% & -78.8\% \\
LiH cmplt BK 631g & 1952 & -34.6\% & -60.6\% & {\cellcolor{green}} -86.0\% & -77.6\% \\
H4 cmplt BK ccpvdz & 2199 & -41.9\% & -50.6\% & {\cellcolor{green}} -88.9\% & -79.9\% \\
H2 cmplt JW 631g & 3732 & -36.6\% & -50.9\% & {\cellcolor{green}} -86.7\% & -75.3\% \\
LiH frz JW ccpvdz & 3768 & -39.3\% & -62.8\% & {\cellcolor{green}} -86.9\% & -77.1\% \\
LiH cmplt BK sto3g & 3768 & -39.3\% & -62.8\% & {\cellcolor{green}} -86.9\% & -77.1\% \\
LiH cmplt JW 631g & 3768 & -47.0\% & -62.8\% & {\cellcolor{green}} -86.0\% & -78.3\% \\
NH cmplt P sto3g & 3769 & -34.7\% & -46.6\% & {\cellcolor{green}} -87.1\% & -76.4\% \\
LiH frz BK sto3g & 3769 & -34.7\% & -46.6\% & {\cellcolor{green}} -87.1\% & -76.4\% \\
NH frz P 631g & 3849 & -37.2\% & -50.9\% & {\cellcolor{green}} -86.9\% & -78.8\% \\
CH2 cmplt P sto3g & 3849 & -37.2\% & -50.9\% & {\cellcolor{green}} -86.9\% & -78.8\% \\
H8 cmplt JW sto3g & 4229 & -52.1\% & -56.6\% & {\cellcolor{green}} -87.7\% & -78.9\% \\
H2 cmplt P ccpvtz & 4890 & -50.7\% & -49.6\% & {\cellcolor{green}} -93.7\% & -86.2\% \\
\bottomrule
\end{tabular}
    
    \caption{Entangling depth comparison for UCCSD Ansätze synthesis for different molecules, encodings, and bases. The first column displays the naive entangling gate depth obtained by individually synthesizing each rotation using two CNOT ladders. Other columns display the entangling gate depth gain with respect to that value. The best result of each row is outlined in green.}
    \label{tab:tab_chem_depth_1}
\end{table}

\begin{table}
\begin{tabular}{lrrrrr}
\toprule
 & naive & ph & tket & rdepth & rcount \\
 & depth & depth & depth & depth & depth \\
name &  &  &  &  &  \\
\midrule
H2 cmplt P ccpvtz & 4890 & -50.7\% & -49.6\% & {\cellcolor{green}} -93.7\% & -86.2\% \\
H2O frz JW sto3g & 4890 & -50.7\% & -49.6\% & {\cellcolor{green}} -93.7\% & -86.2\% \\
C2H4 frz BK sto3g & 4917 & -45.6\% & -61.2\% & {\cellcolor{green}} -86.8\% & -77.6\% \\
H4 cmplt BK sto3g & 4923 & -37.2\% & -46.3\% & {\cellcolor{green}} -87.3\% & -76.1\% \\
H2 cmplt BK ccpvdz & 5078 & -46.1\% & -38.2\% & {\cellcolor{green}} -94.2\% & -89.6\% \\
H2 cmplt P sto3g & 5078 & -46.1\% & -38.2\% & {\cellcolor{green}} -94.2\% & -89.6\% \\
H2O cmplt JW sto3g & 5175 & -46.5\% & -48.2\% & {\cellcolor{green}} -87.5\% & -77.7\% \\
LiH cmplt P ccpvdz & 5188 & -58.6\% & -50.3\% & {\cellcolor{green}} -93.8\% & -88.4\% \\
LiH frz BK 631g & 5188 & -58.6\% & -50.3\% & {\cellcolor{green}} -93.8\% & -88.4\% \\
H2O frz BK sto3g & 6219 & -46.0\% & -52.5\% & {\cellcolor{green}} -88.6\% & -74.2\% \\
LiH frz JW sto3g & 6240 & -35.9\% & -61.6\% & {\cellcolor{green}} -86.7\% & -80.9\% \\
C2H4 cmplt P sto3g & 6251 & -37.5\% & -43.7\% & {\cellcolor{green}} -87.5\% & -75.4\% \\
LiH frz BK ccpvdz & 8499 & -43.6\% & -53.2\% & {\cellcolor{green}} -85.6\% & -72.4\% \\
LiH cmplt P 631g & 9204 & -45.5\% & -61.6\% & {\cellcolor{green}} -87.2\% & -74.8\% \\
H4 cmplt BK 631g & 9212 & -41.3\% & -51.5\% & {\cellcolor{green}} -87.3\% & -74.6\% \\
H8 cmplt BK sto3g & 9248 & -38.4\% & -45.6\% & {\cellcolor{green}} -86.8\% & -74.4\% \\
NH frz JW 631g & 9264 & -41.5\% & -50.5\% & {\cellcolor{green}} -89.7\% & -74.9\% \\
CH2 cmplt JW sto3g & 9304 & -53.7\% & -62.7\% & {\cellcolor{green}} -87.2\% & -81.6\% \\
CH2 cmplt BK sto3g & 16934 & -52.0\% & -55.4\% & {\cellcolor{green}} -86.8\% & -71.5\% \\
C2H4 frz P sto3g & 16996 & -48.5\% & -66.6\% & {\cellcolor{green}} -87.0\% & -73.5\% \\
H4 cmplt P sto3g & 17031 & -40.0\% & -46.4\% & {\cellcolor{green}} -86.9\% & -73.9\% \\
CH2 frz JW sto3g & 18200 & -55.2\% & -45.2\% & {\cellcolor{green}} -92.9\% & -92.3\% \\
H2 cmplt BK ccpvtz & 21578 & -54.6\% & -26.2\% & {\cellcolor{green}} -94.8\% & -93.5\% \\
H4 cmplt P ccpvdz & 21804 & -66.1\% & -36.8\% & {\cellcolor{green}} -95.4\% & -92.5\% \\
H2 cmplt BK sto3g & 22492 & -49.7\% & -49.6\% & {\cellcolor{green}} -92.4\% & -75.4\% \\
\bottomrule
\end{tabular}
\caption{See table \ref{tab:tab_chem_depth_1} for details}
    \label{tab:tab_chem_depth_2}
\end{table}
\begin{table}
\begin{tabular}{lrrrrr}
\toprule
 & naive & ph & tket & rdepth & rcount \\
 & depth & depth & depth & depth & depth \\
name &  &  &  &  &  \\
\midrule
H2 cmplt BK sto3g & 22492 & -49.7\% & -49.6\% & {\cellcolor{green}} -92.4\% & -75.4\% \\
H2O cmplt BK sto3g & 22852 & -46.0\% & -46.5\% & {\cellcolor{green}} -92.9\% & -83.1\% \\
H4 cmplt JW sto3g & 22948 & -59.0\% & -57.0\% & {\cellcolor{green}} -91.5\% & -79.7\% \\
H2O cmplt BK 631g & 30988 & -43.0\% & -46.5\% & {\cellcolor{green}} -85.9\% & -72.2\% \\
LiH frz P 631g & 31028 & -53.3\% & -59.4\% & {\cellcolor{green}} -84.9\% & -71.5\% \\
NH cmplt BK 631g & 31966 & -50.8\% & -50.9\% & {\cellcolor{green}} -86.6\% & -71.8\% \\
H2O frz JW 631g & 51383 & -63.4\% & -40.1\% & {\cellcolor{green}} -93.1\% & -92.8\% \\
H2 cmplt BK 631g & 57485 & -53.4\% & -60.9\% & {\cellcolor{green}} -85.6\% & -71.7\% \\
NH cmplt JW 631g & 57528 & -43.7\% & -46.4\% & {\cellcolor{green}} -84.7\% & -69.8\% \\
LiH cmplt P sto3g & 58268 & -52.1\% & -52.1\% & {\cellcolor{green}} -85.4\% & -70.3\% \\
LiH frz P ccpvdz & 61458 & -59.7\% & -10.7\% & {\cellcolor{green}} -94.4\% & -89.1\% \\
CH2 frz BK sto3g & 61844 & -70.3\% & -20.3\% & {\cellcolor{green}} -95.2\% & -94.0\% \\
H4 cmplt JW 631g & 76348 & -56.9\% & -57.8\% & {\cellcolor{green}} -84.6\% & -70.3\% \\
H2O frz P 631g & 77060 & -44.9\% & -50.1\% & {\cellcolor{green}} -85.2\% & -69.0\% \\
LiH cmplt JW ccpvdz & 77084 & -54.2\% & -67.6\% & {\cellcolor{green}} -84.1\% & -75.0\% \\
C2H4 cmplt BK sto3g & 83368 & -52.8\% & -48.5\% & {\cellcolor{green}} -91.5\% & -81.2\% \\
H4 cmplt P 631g & 94738 & -56.2\% & -53.4\% & {\cellcolor{green}} -91.0\% & -82.9\% \\
H8 cmplt P sto3g & 95542 & -52.5\% & -43.0\% & {\cellcolor{green}} -93.7\% & -83.9\% \\
NH cmplt JW sto3g & 95688 & -65.9\% & -51.7\% & {\cellcolor{green}} -92.6\% & -83.2\% \\
NH frz BK sto3g & 100048 & -53.4\% & -62.4\% & {\cellcolor{green}} -86.3\% & -70.9\% \\
NH frz BK 631g & 101389 & -45.7\% & -43.1\% & {\cellcolor{green}} -85.7\% & -70.8\% \\
H2O frz P sto3g & 101639 & -54.7\% & -49.9\% & {\cellcolor{green}} -85.5\% & -71.1\% \\
NH frz JW sto3g & 108700 & -53.0\% & -45.3\% & {\cellcolor{green}} -93.5\% & -81.7\% \\
LiH frz JW 631g & 108816 & -66.5\% & -55.2\% & {\cellcolor{green}} -92.7\% & -81.6\% \\
H2 cmplt JW sto3g & 124657 & -51.7\% & -47.5\% & {\cellcolor{green}} -84.4\% & -69.1\% \\
NH cmplt P 631g & 125861 & -45.8\% & -45.2\% & {\cellcolor{green}} -84.6\% & -68.1\% \\
CH2 frz P sto3g & 126199 & -55.2\% & -62.8\% & {\cellcolor{green}} -84.9\% & -70.2\% \\
NH cmplt BK sto3g & 176810 & -48.4\% & -53.0\% & {\cellcolor{green}} -83.0\% & -66.5\% \\
H2 cmplt JW ccpvtz & 184100 & -53.1\% & -67.7\% & {\cellcolor{green}} -84.0\% & -66.7\% \\
H2 cmplt P 631g & 184700 & -45.8\% & -44.5\% & {\cellcolor{green}} -84.2\% & -68.5\% \\
\bottomrule
\end{tabular}
\caption{See table \ref{tab:tab_chem_depth_1} for details}
    \label{tab:tab_chem_depth_3}
\end{table}


==> table_new_2.tex <==
\begin{table}[]
    \centering

\begin{tabular}{lrrrrr}
\toprule
 & naive & ph & tket & rdepth & rcount \\
 & count & count & count & count & count \\
name &  &  &  &  &  \\
\midrule
LiH cmplt JW sto3g & 38 & -31.5\% & -52.6\% & -68.4\% & {\cellcolor{green}} -71.0\% \\
LiH frz P sto3g & 38 & -31.5\% & -57.8\% & -71.0\% & {\cellcolor{green}} -73.6\% \\
H2O cmplt P sto3g & 56 & -28.5\% & -60.7\% & {\cellcolor{green}} -78.5\% & {\cellcolor{green}} -78.5\% \\
C2H4 cmplt JW sto3g & 630 & -54.7\% & -67.6\% & {\cellcolor{green}} -82.6\% & -80.3\% \\
H2 cmplt P ccpvdz & 666 & -53.1\% & -62.0\% & -78.3\% & {\cellcolor{green}} -84.9\% \\
LiH cmplt BK ccpvdz & 768 & -61.8\% & -73.8\% & -82.1\% & {\cellcolor{green}} -85.5\% \\
H2 cmplt JW ccpvdz & 1448 & -61.8\% & -66.5\% & {\cellcolor{green}} -83.0\% & -82.1\% \\
H2O cmplt JW 631g & 1316 & -53.4\% & -64.5\% & -79.4\% & {\cellcolor{green}} -82.1\% \\
C2H4 frz JW sto3g & 1440 & -56.6\% & -71.4\% & -79.7\% & {\cellcolor{green}} -82.3\% \\
H2O cmplt P 631g & 1442 & -64.0\% & -69.6\% & -85.7\% & {\cellcolor{green}} -89.7\% \\
H2O frz BK 631g & 1616 & -69.3\% & -76.3\% & -83.7\% & {\cellcolor{green}} -88.3\% \\
NH frz P sto3g & 1316 & -59.8\% & -65.9\% & -76.5\% & {\cellcolor{green}} -80.6\% \\
H4 cmplt JW ccpvdz & 3700 & -59.6\% & -64.8\% & -76.4\% & {\cellcolor{green}} -81.0\% \\
LiH cmplt BK 631g & 3896 & -63.0\% & -75.7\% & -77.0\% & {\cellcolor{green}} -81.6\% \\
H4 cmplt BK ccpvdz & 4178 & -67.4\% & -71.3\% & -81.7\% & {\cellcolor{green}} -82.1\% \\
H2 cmplt JW 631g & 7640 & -65.4\% & -72.1\% & -72.9\% & {\cellcolor{green}} -81.7\% \\
LiH frz JW ccpvdz & 8064 & -67.8\% & -78.6\% & -75.2\% & {\cellcolor{green}} -80.1\% \\
LiH cmplt BK sto3g & 8064 & -67.8\% & -78.6\% & -75.2\% & {\cellcolor{green}} -80.1\% \\
LiH cmplt JW 631g & 8064 & -72.0\% & -78.6\% & -72.3\% & {\cellcolor{green}} -81.4\% \\
NH cmplt P sto3g & 7796 & -64.1\% & -70.2\% & -74.0\% & {\cellcolor{green}} -80.7\% \\
LiH frz BK sto3g & 7796 & -64.1\% & -70.2\% & -74.0\% & {\cellcolor{green}} -80.7\% \\
NH frz P 631g & 8004 & -68.2\% & -73.4\% & -73.5\% & {\cellcolor{green}} -80.9\% \\
CH2 cmplt P sto3g & 8004 & -68.2\% & -73.4\% & -73.5\% & {\cellcolor{green}} -80.9\% \\
H8 cmplt JW sto3g & 8680 & -75.2\% & -75.8\% & -74.7\% & {\cellcolor{green}} -84.4\% \\
\bottomrule
\end{tabular}
    
    \caption{Entangling count comparison for UCCSD Ansätze synthesis for different molecules, encodings, and bases. The first column displays the naive entangling gate count obtained by individually synthesizing each rotation using two CNOT ladders. Other columns display the entangling gate count gain with respect to that value. The best result of each row is outlined in green.}
    \label{tab:tab_chem_1}
\end{table}

\begin{table}[]
    \centering

\begin{tabular}{lrrrrr}
\toprule
 & naive & ph & tket & rdepth & rcount \\
 & count & count & count & count & count \\
name &  &  &  &  &  \\
\midrule
H2 cmplt P ccpvtz & 11344 & -78.5\% & -77.6\% & -84.0\% & {\cellcolor{green}} -92.9\% \\
H2O frz JW sto3g & 11344 & -78.5\% & -77.6\% & -84.0\% & {\cellcolor{green}} -92.9\% \\
C2H4 frz BK sto3g & 10344 & -70.0\% & -76.2\% & -73.7\% & {\cellcolor{green}} -80.4\% \\
H4 cmplt BK sto3g & 9938 & -64.8\% & -67.5\% & -72.3\% & {\cellcolor{green}} -80.5\% \\
H2 cmplt BK ccpvdz & 13878 & -79.9\% & -76.4\% & -88.4\% & {\cellcolor{green}} -94.1\% \\
H2 cmplt P sto3g & 13878 & -79.9\% & -76.4\% & -88.4\% & {\cellcolor{green}} -94.1\% \\
H2O cmplt JW sto3g & 10228 & -70.8\% & -68.2\% & -72.5\% & {\cellcolor{green}} -81.4\% \\
LiH cmplt P ccpvdz & 14616 & -84.3\% & -81.6\% & -87.0\% & {\cellcolor{green}} -94.8\% \\
LiH frz BK 631g & 14616 & -84.3\% & -81.6\% & -87.0\% & {\cellcolor{green}} -94.8\% \\
H2O frz BK sto3g & 13108 & -70.4\% & -73.6\% & -74.1\% & {\cellcolor{green}} -77.9\% \\
LiH frz JW sto3g & 14360 & -68.6\% & -79.9\% & -69.9\% & {\cellcolor{green}} -80.3\% \\
C2H4 cmplt P sto3g & 14020 & -67.9\% & -70.5\% & -72.2\% & {\cellcolor{green}} -79.7\% \\
LiH frz BK ccpvdz & 17924 & -69.7\% & -74.3\% & -57.6\% & {\cellcolor{green}} -84.5\% \\
LiH cmplt P 631g & 21072 & -72.1\% & -78.9\% & -70.2\% & {\cellcolor{green}} -80.3\% \\
H4 cmplt BK 631g & 19574 & -69.1\% & -69.2\% & -67.7\% & {\cellcolor{green}} -79.2\% \\
H8 cmplt BK sto3g & 20514 & -67.8\% & -68.0\% & -68.2\% & {\cellcolor{green}} -79.3\% \\
NH frz JW 631g & 22316 & -72.4\% & -76.1\% & -76.0\% & {\cellcolor{green}} -78.3\% \\
CH2 cmplt JW sto3g & 23200 & -79 & {\cellcolor{green}} -81.9\% & -68.7\% & -80.3\% \\
CH2 cmplt BK sto3g & 37272 & -74.9\% & -74.1\% & -60.3\% & {\cellcolor{green}} -76.2\% \\
C2H4 frz P sto3g & 42368 & -75.2\% & {\cellcolor{green}} -80.5\% & -66.3\% & -79.7\% \\
H4 cmplt P sto3g & 41432 & -70.8\% & -69.6\% & -64.8\% & {\cellcolor{green}} -78.6\% \\
CH2 frz JW sto3g & 49880 & -83.4\% & -79.5\% & -64.7\% & {\cellcolor{green}} -94.8\% \\
H2 cmplt BK ccpvtz & 86598 & -88.5\% & -81.1\% & -82.2\% & {\cellcolor{green}} -97.0\% \\
H4 cmplt P ccpvdz & 89080 & -91.1\% & -84.1\% & -86.1\% & {\cellcolor{green}} -97.1\% \\
\bottomrule
\end{tabular}
\caption{See table \ref{tab:tab_chem_1} for details}
    \label{tab:tab_chem_2}
\end{table}

\begin{table}[]
    \centering

\begin{tabular}{lrrrrr}
\toprule
 & naive & ph & tket & rdepth & rcount \\
 & count & count & count & count & count \\
name &  &  &  &  &  \\
\midrule
H2 cmplt BK sto3g & 53450 & -77.6\% & -76.0\% & -76.0\% & {\cellcolor{green}} -88.0\% \\
H2O cmplt BK sto3g & 67270 & -79.1\% & -79.0\% & -82.0\% & {\cellcolor{green}} -91.5\% \\
H4 cmplt JW sto3g & 69144 & -84.5\% & -83.4\% & -78.6\% & {\cellcolor{green}} -93.4\% \\
H2O cmplt BK 631g & 86650 & -76.0\% & -75.0\% & -56.1\% & {\cellcolor{green}} -76.1\% \\
LiH frz P 631g & 88536 & -80.7\% & {\cellcolor{green}} -82.2\% & -52.6\% & -75.8\% \\
NH cmplt BK 631g & 75664 & {\cellcolor{green}} -77.4\% & -72.3\% & -51.0\% & -73.4\% \\
H2O frz JW 631g & 168986 & -88.8\% & -81.6\% & -49.6\% & {\cellcolor{green}} -96.4\% \\
H2 cmplt BK 631g & 173264 & -81.0\% & {\cellcolor{green}} -82.7\% & -53.2\% & -75.8\% \\
NH cmplt JW 631g & 170666 & {\cellcolor{green}} -77.0\% & -74.6\% & -48.1\% & -75.4\% \\
LiH cmplt P sto3g & 149540 & {\cellcolor{green}} -78.9\% & -73.8\% & -43.0\% & -72.3\% \\
LiH frz P ccpvdz & 335178 & -92.5\% & -83.3\% & -75.5\% & {\cellcolor{green}} -98.1\% \\
CH2 frz BK sto3g & 341280 & -94.2\% & -85.3\% & -79.7\% & {\cellcolor{green}} -98.2\% \\
H4 cmplt JW 631g & 216216 & {\cellcolor{green}} -82.6\% & -80.9\% & -39.6\% & -74.4\% \\
H2O frz P 631g & 241664 & -78.7\% & {\cellcolor{green}} -78.7\% & -48.3\% & -74.0\% \\
LiH cmplt JW ccpvdz & 244992 & -82.2\% & {\cellcolor{green}} -85.7\% & -43.9\% & -74.8\% \\
C2H4 cmplt BK sto3g & 230810 & -81.6\% & -78.5\% & -55.1\% & {\cellcolor{green}} -93.5\% \\
H4 cmplt P 631g & 276768 & -83.8\% & -81.8\% & -51.6\% & {\cellcolor{green}} -93.1\% \\
H8 cmplt P sto3g & 401046 & -87.2\% & -84.4\% & -79.3\% & {\cellcolor{green}} -95.4\% \\
NH cmplt JW sto3g & 407320 & -90.9\% & -87.0\% & -74.6\% & {\cellcolor{green}} -96.0\% \\
NH frz BK sto3g & 312096 & -81.1\% & {\cellcolor{green}} -82.1\% & -52.4\% & -75.5\% \\
NH frz BK 631g & 309068 & {\cellcolor{green}} -77.8\% & -71.5\% & -48.4\% & -75.3\% \\
H2O frz P sto3g & 260656 & {\cellcolor{green}} -79.5\% & -70.6\% & -37.5\% & -72.0\% \\
NH frz JW sto3g & 472132 & -87.7\% & -85.3\% & -76.8\% & {\cellcolor{green}} -96.0\% \\
LiH frz JW 631g & 479136 & -91.3\% & -88.2\% & -73.7\% & {\cellcolor{green}} -96.5\% \\
H2 cmplt JW sto3g & 317504 & {\cellcolor{green}} -78.2\% & -67.4\% & -25.4\% & -66.3\% \\
NH cmplt P 631g & 410000 & {\cellcolor{green}} -79.4\% & -75.1\% & -42.6\% & -74.0\% \\
CH2 frz P sto3g & 414240 & -82.6\% & {\cellcolor{green}} -84.4\% & -44.2\% & -74.5\% \\
NH cmplt BK sto3g & 488548 & {\cellcolor{green}} -78.0\% & -73.7\% & -17.7\% & -66.1\% \\
H2 cmplt JW ccpvtz & 640768 & -82.6\% & {\cellcolor{green}} -86.3\% & -39.0\% & -73.8\% \\
H2 cmplt P 631g & 636668 & {\cellcolor{green}} -80.0\% & -75.5\% & -39.5\% & -74.1\% \\
\bottomrule
\end{tabular}
\caption{See table \ref{tab:tab_chem_1} for details}
    \label{tab:tab_chem_3}
\end{table}

\begin{table}[]
    \centering

\begin{tabular}{lrrrrr}
\toprule
 & naive & ph & tket & rdepth & rcount \\
 & depth & depth & depth & depth & depth \\
name &  &  &  &  &  \\
\midrule
LiH cmplt JW sto3g & 32 & -25 & -46.8\% & {\cellcolor{green}} -68.7\% & {\cellcolor{green}} -68.7\% \\
LiH frz P sto3g & 34 & -29.4\% & -58.8\% & -67.6\% & {\cellcolor{green}} -70.5\% \\
H2O cmplt P sto3g & 36 & 5.5\% & -50 & {\cellcolor{green}} -72.2\% & {\cellcolor{green}} -72.2\% \\
C2H4 cmplt JW sto3g & 405 & -33.3\% & -53.8\% & {\cellcolor{green}} -85.6\% & -75.5\% \\
H2 cmplt P ccpvdz & 412 & -26.6\% & -43.2\% & {\cellcolor{green}} -84.9\% & -82.0\% \\
LiH cmplt BK ccpvdz & 436 & -36.9\% & -58.0\% & {\cellcolor{green}} -85.7\% & -80.9\% \\
H2 cmplt JW ccpvdz & 790 & -32.0\% & -42.6\% & {\cellcolor{green}} -87.8\% & -75.5\% \\
H2O cmplt JW 631g & 800 & -29.2\% & -50 & {\cellcolor{green}} -86.1\% & -78.6\% \\
C2H4 frz JW sto3g & 812 & -31.1\% & -60.4\% & {\cellcolor{green}} -85.8\% & -77.3\% \\
H2O cmplt P 631g & 812 & -37.9\% & -48.1\% & {\cellcolor{green}} -90.7\% & -87.6\% \\
H2O frz BK 631g & 832 & -44.2\% & -57.4\% & {\cellcolor{green}} -88.7\% & -83.1\% \\
NH frz P sto3g & 838 & -40.6\% & -53.4\% & {\cellcolor{green}} -86.2\% & -78.4\% \\
H4 cmplt JW ccpvdz & 1947 & -31.0\% & -43.4\% & {\cellcolor{green}} -86.1\% & -74.1\% \\
LiH cmplt BK 631g & 1952 & -34.6\% & -60.6\% & {\cellcolor{green}} -86.0\% & -75 \\
H4 cmplt BK ccpvdz & 2199 & -41.9\% & -50.6\% & {\cellcolor{green}} -88.9\% & -76.3\% \\
H2 cmplt JW 631g & 3732 & -36.6\% & -50.9\% & {\cellcolor{green}} -86.7\% & -74.3\% \\
LiH frz JW ccpvdz & 3768 & -39.3\% & -62.8\% & {\cellcolor{green}} -86.9\% & -70.7\% \\
LiH cmplt BK sto3g & 3768 & -39.3\% & -62.8\% & {\cellcolor{green}} -86.9\% & -70.7\% \\
LiH cmplt JW 631g & 3768 & -47.0\% & -62.8\% & {\cellcolor{green}} -86.0\% & -72.2\% \\
NH cmplt P sto3g & 3769 & -34.7\% & -46.6\% & {\cellcolor{green}} -87.1\% & -73.2\% \\
LiH frz BK sto3g & 3769 & -34.7\% & -46.6\% & {\cellcolor{green}} -87.1\% & -73.2\% \\
NH frz P 631g & 3849 & -37.2\% & -50.9\% & {\cellcolor{green}} -86.9\% & -72.8\% \\
CH2 cmplt P sto3g & 3849 & -37.2\% & -50.9\% & {\cellcolor{green}} -86.9\% & -72.8\% \\
H8 cmplt JW sto3g & 4229 & -52.1\% & -56.6\% & {\cellcolor{green}} -87.7\% & -79.0\% \\
\bottomrule
\end{tabular}
    
    \caption{Entangling depth comparison for UCCSD Ansätze synthesis for different molecules, encodings, and bases. The first column displays the naive entangling gate depth obtained by individually synthesizing each rotation using two CNOT ladders. Other columns display the entangling gate depth gain with respect to that value. The best result of each row is outlined in green.}
    \label{tab:tab_chem_depth_1}
\end{table}

\begin{table}[]
    \centering

\begin{tabular}{lrrrrr}
\toprule
 & naive & ph & tket & rdepth & rcount \\
 & depth & depth & depth & depth & depth \\
name &  &  &  &  &  \\
\midrule
H2 cmplt P ccpvtz & 4890 & -50.7\% & -49.6\% & {\cellcolor{green}} -93.7\% & -89.8\% \\
H2O frz JW sto3g & 4890 & -50.7\% & -49.6\% & {\cellcolor{green}} -93.7\% & -89.8\% \\
C2H4 frz BK sto3g & 4917 & -45.6\% & -61.2\% & {\cellcolor{green}} -86.8\% & -72.8\% \\
H4 cmplt BK sto3g & 4923 & -37.2\% & -46.3\% & {\cellcolor{green}} -87.3\% & -73.5\% \\
H2 cmplt BK ccpvdz & 5078 & -46.1\% & -38.2\% & {\cellcolor{green}} -94.2\% & -90.8\% \\
H2 cmplt P sto3g & 5078 & -46.1\% & -38.2\% & {\cellcolor{green}} -94.2\% & -90.8\% \\
H2O cmplt JW sto3g & 5175 & -46.5\% & -48.2\% & {\cellcolor{green}} -87.5\% & -75.8\% \\
LiH cmplt P ccpvdz & 5188 & -58.6\% & -50.3\% & {\cellcolor{green}} -93.8\% & -90.5\% \\
LiH frz BK 631g & 5188 & -58.6\% & -50.3\% & {\cellcolor{green}} -93.8\% & -90.5\% \\
H2O frz BK sto3g & 6219 & -46.0\% & -52.5\% & {\cellcolor{green}} -88.6\% & -69.2\% \\
LiH frz JW sto3g & 6240 & -35.9\% & -61.6\% & {\cellcolor{green}} -86.7\% & -69.6\% \\
C2H4 cmplt P sto3g & 6251 & -37.5\% & -43.7\% & {\cellcolor{green}} -87.5\% & -70.3\% \\
LiH frz BK ccpvdz & 8499 & -43.6\% & -53.2\% & {\cellcolor{green}} -85.6\% & -79.2\% \\
LiH cmplt P 631g & 9204 & -45.5\% & -61.6\% & {\cellcolor{green}} -87.2\% & -70.7\% \\
H4 cmplt BK 631g & 9212 & -41.3\% & -51.5\% & {\cellcolor{green}} -87.3\% & -71.2\% \\
H8 cmplt BK sto3g & 9248 & -38.4\% & -45.6\% & {\cellcolor{green}} -86.8\% & -69.9\% \\
NH frz JW 631g & 9264 & -41.5\% & -50.5\% & {\cellcolor{green}} -89.7\% & -66.3\% \\
CH2 cmplt JW sto3g & 9304 & -53.7\% & -62.7\% & {\cellcolor{green}} -87.2\% & -68.6\% \\
CH2 cmplt BK sto3g & 16934 & -52.0\% & -55.4\% & {\cellcolor{green}} -86.8\% & -66.7\% \\
C2H4 frz P sto3g & 16996 & -48.5\% & -66.6\% & {\cellcolor{green}} -87.0\% & -67.7\% \\
H4 cmplt P sto3g & 17031 & -40.0\% & -46.4\% & {\cellcolor{green}} -86.9\% & -66.9\% \\
CH2 frz JW sto3g & 18200 & -55.2\% & -45.2\% & {\cellcolor{green}} -92.9\% & -91.5\% \\
H2 cmplt BK ccpvtz & 21578 & -54.6\% & -26.2\% & {\cellcolor{green}} -94.8\% & -93.6\% \\
H4 cmplt P ccpvdz & 21804 & -66.1\% & -36.8\% & {\cellcolor{green}} -95.4\% & -92.9\% \\
\bottomrule
\end{tabular}
\caption{See table \ref{tab:tab_chem_depth_1} for details}
    \label{tab:tab_chem_depth_2}
\end{table}
\begin{table}[]
    \centering

\begin{tabular}{lrrrrr}
\toprule
 & naive & ph & tket & rdepth & rcount \\
 & depth & depth & depth & depth & depth \\
name &  &  &  &  &  \\
\midrule
H2 cmplt BK sto3g & 22492 & -49.7\% & -49.6\% & {\cellcolor{green}} -92.4\% & -83.8\% \\
H2O cmplt BK sto3g & 22852 & -46.0\% & -46.5\% & {\cellcolor{green}} -92.9\% & -84.6\% \\
H4 cmplt JW sto3g & 22948 & -59.0\% & -57.0\% & {\cellcolor{green}} -91.5\% & -88.0\% \\
H2O cmplt BK 631g & 30988 & -43.0\% & -46.5\% & {\cellcolor{green}} -85.9\% & -59.2\% \\
LiH frz P 631g & 31028 & -53.3\% & -59.4\% & {\cellcolor{green}} -84.9\% & -58.2\% \\
NH cmplt BK 631g & 31966 & -50.8\% & -50.9\% & {\cellcolor{green}} -86.6\% & -61.8\% \\
H2O frz JW 631g & 51383 & -63.4\% & -40.1\% & {\cellcolor{green}} -93.1\% & -92.5\% \\
H2 cmplt BK 631g & 57485 & -53.4\% & -60.9\% & {\cellcolor{green}} -85.6\% & -56.7\% \\
NH cmplt JW 631g & 57528 & -43.7\% & -46.4\% & {\cellcolor{green}} -84.7\% & -57.0\% \\
LiH cmplt P sto3g & 58268 & -52.1\% & -52.1\% & {\cellcolor{green}} -85.4\% & -58.2\% \\
LiH frz P ccpvdz & 61458 & -59.7\% & -10.7\% & {\cellcolor{green}} -94.4\% & -93.7\% \\
CH2 frz BK sto3g & 61844 & -70.3\% & -20.3\% & {\cellcolor{green}} -95.2\% & -93.9\% \\
H4 cmplt JW 631g & 76348 & -56.9\% & -57.8\% & {\cellcolor{green}} -84.6\% & -59.2\% \\
H2O frz P 631g & 77060 & -44.9\% & -50.1\% & {\cellcolor{green}} -85.2\% & -53.1\% \\
LiH cmplt JW ccpvdz & 77084 & -54.2\% & -67.6\% & {\cellcolor{green}} -84.1\% & -53.6\% \\
C2H4 cmplt BK sto3g & 83368 & -52.8\% & -48.5\% & {\cellcolor{green}} -91.5\% & -90.9\% \\
H4 cmplt P 631g & 94738 & -56.2\% & -53.4\% & {\cellcolor{green}} -91.0\% & -89.7\% \\
H8 cmplt P sto3g & 95542 & -52.5\% & -43.0\% & {\cellcolor{green}} -93.7\% & -90.4\% \\
NH cmplt JW sto3g & 95688 & -65.9\% & -51.7\% & {\cellcolor{green}} -92.6\% & -90.6\% \\
NH frz BK sto3g & 100048 & -53.4\% & -62.4\% & {\cellcolor{green}} -86.3\% & -56.1\% \\
NH frz BK 631g & 101389 & -45.7\% & -43.1\% & {\cellcolor{green}} -85.7\% & -56.6\% \\
H2O frz P sto3g & 101639 & -54.7\% & -49.9\% & {\cellcolor{green}} -85.5\% & -58.5\% \\
NH frz JW sto3g & 108700 & -53.0\% & -45.3\% & {\cellcolor{green}} -93.5\% & -90.6\% \\
LiH frz JW 631g & 108816 & -66.5\% & -55.2\% & {\cellcolor{green}} -92.7\% & -92.1\% \\
H2 cmplt JW sto3g & 124657 & -51.7\% & -47.5\% & {\cellcolor{green}} -84.4\% & -51.6\% \\
NH cmplt P 631g & 125861 & -45.8\% & -45.2\% & {\cellcolor{green}} -84.6\% & -52.5\% \\
CH2 frz P sto3g & 126199 & -55.2\% & -62.8\% & {\cellcolor{green}} -84.9\% & -52.9\% \\
NH cmplt BK sto3g & 176810 & -48.4\% & -53.0\% & {\cellcolor{green}} -83.0\% & -48.7\% \\
H2 cmplt JW ccpvtz & 184100 & -53.1\% & -67.7\% & {\cellcolor{green}} -84.0\% & -50.0\% \\
H2 cmplt P 631g & 184700 & -45.8\% & -44.5\% & {\cellcolor{green}} -84.2\% & -51.0\% \\
\bottomrule
\end{tabular}

\caption{See table \ref{tab:tab_chem_depth_1} for details}
    \label{tab:tab_chem_depth_3}
\end{table}

==> table_new_3.tex <==
\begin{table}[]
    \centering

\begin{tabular}{lrrrrr}
\toprule
 & naive & ph & tket & rdepth & rcount \\
 & count & count & count & count & count \\
name &  &  &  &  &  \\
\midrule
LiH cmplt JW sto3g & 38 & -31.5\% & -52.6\% & {\cellcolor{green}} -68.4\% & {\cellcolor{green}} -68.4\% \\
LiH frz P sto3g & 38 & -31.5\% & -57.8\% & {\cellcolor{green}} -76.3\% & -73.6\% \\
H2O cmplt P sto3g & 630 & -54.7\% & -67.6\% & -83.4\% & {\cellcolor{green}} -86.0\% \\
C2H4 cmplt JW sto3g & 666 & -53.1\% & -62.0\% & {\cellcolor{green}} -80.4\% & -80.0\% \\
H2 cmplt P ccpvdz & 768 & -61.8\% & -73.8\% & -86.7\% & {\cellcolor{green}} -87.8\% \\
LiH cmplt BK ccpvdz & 1448 & -61.8\% & -66.5\% & -82.5\% & {\cellcolor{green}} -85.2\% \\
H2 cmplt JW ccpvdz & 1316 & -53.4\% & -64.5\% & -78.5\% & {\cellcolor{green}} -85.1\% \\
H2O cmplt JW 631g & 1442 & -64.0\% & -69.6\% & -77.8\% & {\cellcolor{green}} -88.1\% \\
C2H4 frz JW sto3g & 1440 & -56.6\% & -71.4\% & -79.8\% & {\cellcolor{green}} -84.3\% \\
H2O cmplt P 631g & 1616 & -69.3\% & -76.3\% & -82.6\% & {\cellcolor{green}} -90.1\% \\
NH frz P sto3g & 1316 & -59.8\% & -65.9\% & -76.6\% & {\cellcolor{green}} -82.2\% \\
H4 cmplt JW ccpvdz & 3700 & -59.6\% & -64.8\% & -75.1\% & {\cellcolor{green}} -82.3\% \\
LiH cmplt BK 631g & 3896 & -63.0\% & -75.7\% & -78.1\% & {\cellcolor{green}} -85.0\% \\
H4 cmplt BK ccpvdz & 4178 & -67.4\% & -71.3\% & -80.2\% & {\cellcolor{green}} -84.6\% \\
H2 cmplt JW 631g & 7640 & -65.4\% & -72.1\% & -71.8\% & {\cellcolor{green}} -80.7\% \\
LiH frz JW ccpvdz & 8064 & -72.0\% & -78.6\% & -75.8\% & {\cellcolor{green}} -82.5\% \\
LiH cmplt BK sto3g & 7796 & -64.1\% & -70.2\% & -72.8\% & {\cellcolor{green}} -80.7\% \\
LiH frz BK sto3g & 8064 & -67.8\% & -78.6\% & -74.2\% & {\cellcolor{green}} -83.0\% \\
NH frz P 631g & 8004 & -68.2\% & -73.4\% & -75.2\% & {\cellcolor{green}} -81.1\% \\
H8 cmplt JW sto3g & 8004 & -68.2\% & -73.4\% & -75.2\% & {\cellcolor{green}} -81.1\% \\
H2 cmplt P ccpvtz & 8680 & -75.2\% & -75.8\% & -79.2\% & {\cellcolor{green}} -83.0\% \\
C2H4 frz BK sto3g & 11344 & -78.5\% & -77.6\% & -82.7\% & {\cellcolor{green}} -92.8\% \\
H4 cmplt BK sto3g & 11344 & -78.5\% & -77.6\% & -82.7\% & {\cellcolor{green}} -92.8\% \\
H2 cmplt BK ccpvdz & 10344 & -70.0\% & -76.2\% & -74.4\% & {\cellcolor{green}} -82.2\% \\
\bottomrule
\end{tabular}
    
    \caption{Entangling count comparison for UCCSD Ansätze synthesis for different molecules, encodings, and bases. The first column displays the naive entangling gate count obtained by individually synthesizing each rotation using two CNOT ladders. Other columns display the entangling gate count gain with respect to that value. The best result of each row is outlined in green.}
    \label{tab:tab_chem_1}
\end{table}

\begin{table}[]
    \centering

\begin{tabular}{lrrrrr}
\toprule
 & naive & ph & tket & rdepth & rcount \\
 & count & count & count & count & count \\
name &  &  &  &  &  \\
\midrule
H2 cmplt P sto3g & 9938 & -64.5\% & -67.5\% & -74.0\% & {\cellcolor{green}} -80.3\% \\
H2O cmplt JW sto3g & 13878 & -79.9\% & -76.4\% & -86.6\% & {\cellcolor{green}} -94.9\% \\
LiH cmplt P ccpvdz & 10228 & -70.8\% & -68.2\% & -74.9\% & {\cellcolor{green}} -82.6\% \\
LiH frz BK 631g & 14616 & -84.3\% & -81.6\% & -86.4\% & {\cellcolor{green}} -94.6\% \\
H2O frz BK sto3g & 14616 & -84.3\% & -81.6\% & -86.4\% & {\cellcolor{green}} -94.6\% \\
LiH frz JW sto3g & 13108 & -70.4\% & -73.6\% & -71.8\% & {\cellcolor{green}} -80.0\% \\
C2H4 cmplt P sto3g & 14360 & -68.6\% & -79.9\% & -72.7\% & {\cellcolor{green}} -80.3\% \\
LiH frz BK ccpvdz & 14020 & -67.9\% & -70.5\% & -72.1\% & {\cellcolor{green}} -82.4\% \\
LiH cmplt P 631g & 17924 & -69.7\% & -74.3\% & -69.7\% & {\cellcolor{green}} -81.4\% \\
H4 cmplt BK 631g & 19574 & -69.1\% & -69.2\% & -71.3\% & {\cellcolor{green}} -79.5\% \\
H8 cmplt BK sto3g & 21072 & -72.1\% & -78.9\% & -72.7\% & {\cellcolor{green}} -80.6\% \\
NH frz JW 631g & 22316 & -72.4\% & -76.1\% & -78.2\% & {\cellcolor{green}} -80.4\% \\
CH2 cmplt JW sto3g & 23200 & -79 & {\cellcolor{green}} -81.9\% & -69.6\% & -81.0\% \\
CH2 cmplt BK sto3g & 37272 & -74.9\% & -74.1\% & -62.2\% & {\cellcolor{green}} -78.0\% \\
C2H4 frz P sto3g & 42368 & -75.2\% & {\cellcolor{green}} -80.5\% & -68.7\% & -80.0\% \\
H4 cmplt P sto3g & 41432 & -70.8\% & -69.6\% & -68.7\% & {\cellcolor{green}} -79.1\% \\
CH2 frz JW sto3g & 49880 & -83.4\% & -79.5\% & -72.8\% & {\cellcolor{green}} -94.2\% \\
H2 cmplt BK ccpvtz & 86598 & -88.5\% & -81.1\% & -79.1\% & {\cellcolor{green}} -96.8\% \\
H4 cmplt P ccpvdz & 89080 & -91.1\% & -84.1\% & -83.9\% & {\cellcolor{green}} -97.0\% \\
H2 cmplt BK sto3g & 53450 & -77.6\% & -76.0\% & -76.2\% & {\cellcolor{green}} -91.3\% \\
H2O cmplt BK sto3g & 67270 & -79.1\% & -79.0\% & -79.4\% & {\cellcolor{green}} -91.2\% \\
H4 cmplt JW sto3g & 86650 & -76.0\% & -75.0\% & -55.5\% & {\cellcolor{green}} -77.2\% \\
H2O cmplt BK 631g & 88536 & -80.7\% & {\cellcolor{green}} -82.2\% & -63.0\% & -77.0\% \\
NH cmplt BK 631g & 75664 & {\cellcolor{green}} -77.4\% & -72.3\% & -51.4\% & -74.3\% \\
\bottomrule
\end{tabular}
\caption{See table \ref{tab:tab_chem_1} for details}
    \label{tab:tab_chem_2}
\end{table}


\begin{table}[]
    \centering

\begin{tabular}{lrrrrr}
\toprule
 & naive & ph & tket & rdepth & rcount \\
 & count & count & count & count & count \\
name &  &  &  &  &  \\
\midrule
H2O frz JW 631g & 168986 & -88.8\% & -81.6\% & -55.5\% & {\cellcolor{green}} -96.6\% \\
H2 cmplt BK 631g & 173264 & -81.0\% & {\cellcolor{green}} -82.7\% & -55.9\% & -76.7\% \\
NH cmplt JW 631g & 170666 & {\cellcolor{green}} -77.0\% & -74.6\% & -53.3\% & -76.2\% \\
LiH cmplt P sto3g & 149540 & {\cellcolor{green}} -78.9\% & -73.8\% & -47.8\% & -72.8\% \\
LiH frz P ccpvdz & 335178 & -92.5\% & -83.3\% & -74.4\% & {\cellcolor{green}} -98.2\% \\
CH2 frz BK sto3g & 341280 & -94.2\% & -85.3\% & -77.5\% & {\cellcolor{green}} -98.2\% \\
H4 cmplt JW 631g & 244992 & -82.2\% & {\cellcolor{green}} -85.7\% & -50.6\% & -75.3\% \\
LiH cmplt JW ccpvdz & 230810 & -81.6\% & -78.5\% & -58.8\% & {\cellcolor{green}} -94.0\% \\
C2H4 cmplt BK sto3g & 276768 & -83.8\% & -81.8\% & -46.8\% & {\cellcolor{green}} -93.6\% \\
H4 cmplt P 631g & 401046 & -87.2\% & -84.4\% & -77.4\% & {\cellcolor{green}} -96.6\% \\
H8 cmplt P sto3g & 407320 & -90.9\% & -87.0\% & -78.3\% & {\cellcolor{green}} -96.5\% \\
NH cmplt JW sto3g & 312096 & -81.1\% & {\cellcolor{green}} -82.1\% & -50.7\% & -76.6\% \\
NH frz BK sto3g & 309068 & {\cellcolor{green}} -77.8\% & -71.5\% & -56.1\% & -76.0\% \\
NH frz BK 631g & 260656 & {\cellcolor{green}} -79.5\% & -70.6\% & -47.5\% & -71.4\% \\
H2O frz P sto3g & 472132 & -87.7\% & -85.3\% & -74.7\% & {\cellcolor{green}} -96.3\% \\
NH frz JW sto3g & 479136 & -91.3\% & -88.2\% & -79.2\% & {\cellcolor{green}} -96.3\% \\
LiH frz JW 631g & 317504 & {\cellcolor{green}} -78.2\% & -67.4\% & -28.2\% & -67.8\% \\
NH cmplt P 631g & 410000 & {\cellcolor{green}} -79.4\% & -75.1\% & -45.6\% & -75.0\% \\
CH2 frz P sto3g & 414240 & -82.6\% & {\cellcolor{green}} -84.4\% & -44.3\% & -75.2\% \\
NH cmplt BK sto3g & 488548 & {\cellcolor{green}} -78.0\% & -73.7\% & -22.0\% & -66.9\% \\
H2 cmplt JW ccpvtz & 640768 & -82.6\% & {\cellcolor{green}} -86.3\% & -48.2\% & -74.3\% \\
H2 cmplt P 631g & 636668 & {\cellcolor{green}} -80.0\% & -75.5\% & -47.3\% & -74.5\% \\
\bottomrule
\end{tabular}
\caption{See table \ref{tab:tab_chem_1} for details}
    \label{tab:tab_chem_3}
\end{table}


\begin{table}[]
    \centering

\begin{tabular}{lrrrrr}
\toprule
 & naive & ph & tket & rdepth & rcount \\
 & depth & depth & depth & depth & depth \\
name &  &  &  &  &  \\
\midrule
LiH cmplt JW sto3g & 32 & -25 & -46.8\% & {\cellcolor{green}} -68.7\% & -65.6\% \\
LiH frz P sto3g & 33 & -27.2\% & -57.5\% & {\cellcolor{green}} -81.8\% & -69.6\% \\
H2O cmplt P sto3g & 406 & -33.4\% & -53.9\% & {\cellcolor{green}} -88.6\% & -83.2\% \\
C2H4 cmplt JW sto3g & 409 & -26.1\% & -42.7\% & {\cellcolor{green}} -85.0\% & -75.7\% \\
H2 cmplt P ccpvdz & 436 & -36.9\% & -58.0\% & {\cellcolor{green}} -88.9\% & -84.8\% \\
LiH cmplt BK ccpvdz & 783 & -31.4\% & -42.1\% & {\cellcolor{green}} -86.9\% & -81.7\% \\
H2 cmplt JW ccpvdz & 796 & -28.8\% & -49.7\% & {\cellcolor{green}} -85.6\% & -81.2\% \\
H2O cmplt JW 631g & 810 & -37.7\% & -48.0\% & {\cellcolor{green}} -86.7\% & -85.5\% \\
C2H4 frz JW sto3g & 812 & -31.1\% & -60.4\% & {\cellcolor{green}} -86.4\% & -79.3\% \\
H2O cmplt P 631g & 830 & -44.0\% & -57.3\% & {\cellcolor{green}} -87.8\% & {\cellcolor{green}} -87.8\% \\
NH frz P sto3g & 838 & -40.6\% & -53.4\% & {\cellcolor{green}} -85.7\% & -78.8\% \\
H4 cmplt JW ccpvdz & 1944 & -30.9\% & -43.3\% & {\cellcolor{green}} -86.0\% & -77.2\% \\
LiH cmplt BK 631g & 1952 & -34.6\% & -60.6\% & {\cellcolor{green}} -86.5\% & -79.2\% \\
H4 cmplt BK ccpvdz & 2193 & -41.7\% & -50.4\% & {\cellcolor{green}} -88.4\% & -79.6\% \\
H2 cmplt JW 631g & 3727 & -36.5\% & -50.8\% & {\cellcolor{green}} -86.7\% & -73.2\% \\
LiH frz JW ccpvdz & 3764 & -46.9\% & -62.8\% & {\cellcolor{green}} -87.2\% & -74.6\% \\
LiH cmplt BK sto3g & 3766 & -34.6\% & -46.5\% & {\cellcolor{green}} -86.9\% & -72.3\% \\
LiH frz BK sto3g & 3768 & -39.3\% & -62.8\% & {\cellcolor{green}} -87.1\% & -75.9\% \\
NH frz P 631g & 3857 & -37.4\% & -51.0\% & {\cellcolor{green}} -87.5\% & -72.8\% \\
H8 cmplt JW sto3g & 3857 & -37.4\% & -51.0\% & {\cellcolor{green}} -87.5\% & -72.8\% \\
H2 cmplt P ccpvtz & 4225 & -52.0\% & -56.5\% & {\cellcolor{green}} -89.4\% & -75.8\% \\
C2H4 frz BK sto3g & 4867 & -50.5\% & -49.4\% & {\cellcolor{green}} -93.7\% & -89.2\% \\
H4 cmplt BK sto3g & 4867 & -50.5\% & -49.4\% & {\cellcolor{green}} -93.7\% & -89.2\% \\
H2 cmplt BK ccpvdz & 4908 & -45.5\% & -61.1\% & {\cellcolor{green}} -87.5\% & -75.5\% \\
\bottomrule
\end{tabular}

    
    \caption{Entangling depth comparison for UCCSD Ansätze synthesis for different molecules, encodings, and bases. The first column displays the naive entangling gate depth obtained by individually synthesizing each rotation using two CNOT ladders. Other columns display the entangling gate depth gain with respect to that value. The best result of each row is outlined in green.}
    \label{tab:tab_chem_depth_1}
\end{table}


\begin{table}[]
    \centering

\begin{tabular}{lrrrrr}
\toprule
 & naive & ph & tket & rdepth & rcount \\
 & depth & depth & depth & depth & depth \\
name &  &  &  &  &  \\
\midrule
H2 cmplt P sto3g & 4915 & -36.7\% & -46.2\% & {\cellcolor{green}} -87.7\% & -73.7\% \\
H2O cmplt JW sto3g & 5060 & -46.0\% & -37.9\% & {\cellcolor{green}} -94.1\% & -91.8\% \\
LiH cmplt P ccpvdz & 5160 & -46.3\% & -48.1\% & {\cellcolor{green}} -88.3\% & -76.6\% \\
LiH frz BK 631g & 5183 & -58.6\% & -50.3\% & {\cellcolor{green}} -93.9\% & -90.7\% \\
H2O frz BK sto3g & 5183 & -58.6\% & -50.3\% & {\cellcolor{green}} -93.9\% & -90.7\% \\
LiH frz JW sto3g & 6218 & -45.9\% & -52.5\% & {\cellcolor{green}} -88.4\% & -72.3\% \\
C2H4 cmplt P sto3g & 6240 & -35.9\% & -61.6\% & {\cellcolor{green}} -87.7\% & -70.0\% \\
LiH frz BK ccpvdz & 6246 & -37.4\% & -43.7\% & {\cellcolor{green}} -87.8\% & -74.0\% \\
LiH cmplt P 631g & 8412 & -43.0\% & -52.7\% & {\cellcolor{green}} -88.8\% & -74.4\% \\
H4 cmplt BK 631g & 9192 & -41.2\% & -51.4\% & {\cellcolor{green}} -88.3\% & -71.0\% \\
H8 cmplt BK sto3g & 9198 & -45.5\% & -61.6\% & {\cellcolor{green}} -88.2\% & -71.2\% \\
NH frz JW 631g & 9249 & -41.4\% & -50.4\% & {\cellcolor{green}} -90.6\% & -69.4\% \\
CH2 cmplt JW sto3g & 9295 & -53.7\% & -62.6\% & {\cellcolor{green}} -87.8\% & -69.7\% \\
CH2 cmplt BK sto3g & 16774 & -51.6\% & -55.0\% & {\cellcolor{green}} -87.3\% & -68.7\% \\
C2H4 frz P sto3g & 16984 & -48.5\% & -66.6\% & {\cellcolor{green}} -87.9\% & -68.2\% \\
H4 cmplt P sto3g & 16994 & -39.8\% & -46.3\% & {\cellcolor{green}} -88.1\% & -67.1\% \\
CH2 frz JW sto3g & 18176 & -55.1\% & -45.1\% & {\cellcolor{green}} -94.5\% & -92.3\% \\
H2 cmplt BK ccpvtz & 21541 & -54.5\% & -26.1\% & {\cellcolor{green}} -93.9\% & -93.5\% \\
H4 cmplt P ccpvdz & 21795 & -66.1\% & -36.8\% & {\cellcolor{green}} -95.0\% & -93.9\% \\
H2 cmplt BK sto3g & 22383 & -49.4\% & -49.4\% & {\cellcolor{green}} -92.5\% & -88.3\% \\
H2O cmplt BK sto3g & 22809 & -45.9\% & -46.4\% & {\cellcolor{green}} -92.2\% & -84.4\% \\
H4 cmplt JW sto3g & 30935 & -42.9\% & -46.5\% & {\cellcolor{green}} -86.0\% & -61.3\% \\
H2O cmplt BK 631g & 30970 & -53.2\% & -59.3\% & {\cellcolor{green}} -87.5\% & -59.9\% \\
NH cmplt BK 631g & 31739 & -50.4\% & -50.5\% & {\cellcolor{green}} -86.9\% & -62.9\% \\
\bottomrule
\end{tabular}
\caption{See table \ref{tab:tab_chem_depth_1} for details}
    \label{tab:tab_chem_depth_2}
\end{table}

\begin{table}[]
    \centering

\begin{tabular}{lrrrrr}
\toprule
 & naive & ph & tket & rdepth & rcount \\
 & depth & depth & depth & depth & depth \\
name &  &  &  &  &  \\
\midrule
H2O frz JW 631g & 51318 & -63.4\% & -40.0\% & {\cellcolor{green}} -93.9\% & -93.2\% \\
H2 cmplt BK 631g & 57380 & -53.3\% & -60.8\% & {\cellcolor{green}} -86.4\% & -58.5\% \\
NH cmplt JW 631g & 57410 & -43.5\% & -46.3\% & {\cellcolor{green}} -86.0\% & -58.1\% \\
LiH cmplt P sto3g & 58159 & -52.0\% & -52.0\% & {\cellcolor{green}} -86.4\% & -58.1\% \\
LiH frz P ccpvdz & 61396 & -59.6\% & -10.6\% & -94.3\% & {\cellcolor{green}} -94.5\% \\
CH2 frz BK sto3g & 61830 & -70.3\% & -20.3\% & {\cellcolor{green}} -94.8\% & -94.3\% \\
H4 cmplt JW 631g & 77014 & -54.2\% & -67.5\% & {\cellcolor{green}} -85.7\% & -54.6\% \\
LiH cmplt JW ccpvdz & 83151 & -52.7\% & -48.4\% & {\cellcolor{green}} -92.2\% & -91.0\% \\
C2H4 cmplt BK sto3g & 94580 & -56.1\% & -53.3\% & {\cellcolor{green}} -90.7\% & -90.1\% \\
H4 cmplt P 631g & 95435 & -52.4\% & -42.9\% & {\cellcolor{green}} -93.4\% & -92.5\% \\
H8 cmplt P sto3g & 95585 & -65.9\% & -51.6\% & {\cellcolor{green}} -93.5\% & -91.2\% \\
NH cmplt JW sto3g & 99877 & -53.3\% & -62.3\% & {\cellcolor{green}} -86.0\% & -57.3\% \\
NH frz BK sto3g & 101189 & -45.6\% & -43.0\% & {\cellcolor{green}} -87.4\% & -57.2\% \\
NH frz BK 631g & 101374 & -54.6\% & -49.7\% & {\cellcolor{green}} -87.3\% & -57.1\% \\
H2O frz P sto3g & 108634 & -52.9\% & -45.2\% & {\cellcolor{green}} -93.0\% & -91.5\% \\
NH frz JW sto3g & 108764 & -66.5\% & -55.2\% & {\cellcolor{green}} -93.9\% & -91.6\% \\
LiH frz JW 631g & 124158 & -51.5\% & -47.3\% & {\cellcolor{green}} -84.9\% & -53.0\% \\
NH cmplt P 631g & 125613 & -45.7\% & -45.1\% & {\cellcolor{green}} -85.3\% & -53.8\% \\
CH2 frz P sto3g & 126020 & -55.1\% & -62.8\% & {\cellcolor{green}} -85.0\% & -53.7\% \\
NH cmplt BK sto3g & 176403 & -48.3\% & -52.9\% & {\cellcolor{green}} -83.7\% & -49.1\% \\
H2 cmplt JW ccpvtz & 183920 & -53.1\% & -67.6\% & {\cellcolor{green}} -86.0\% & -50.6\% \\
H2 cmplt P 631g & 184436 & -45.8\% & -44.4\% & {\cellcolor{green}} -85.9\% & -51.1\% \\
\bottomrule
\end{tabular}
\caption{See table \ref{tab:tab_chem_depth_1} for details}
    \label{tab:tab_chem_depth_3}
\end{table}

% \begin{table}[]
%     \centering

% \begin{tabular}{lrrrrr}
% \toprule
%  & naive & ph & tket & rdepth & rcount \\
%  & time & time & time & time & time \\
% name &  &  &  &  &  \\
% \midrule
% LiH cmplt JW sto3g & 0.0\% & 1680.2\% & 258.0\% & -96.8\% & {\cellcolor{green}} -99.1\% \\
% LiH frz P sto3g & 0.0\% & 571.7\% & -47.6\% & -98.2\% & {\cellcolor{green}} -99.3\% \\
% H2O cmplt P sto3g & 0.0\% & 1178.9\% & -24.0\% & -91.4\% & {\cellcolor{green}} -97.9\% \\
% C2H4 cmplt JW sto3g & 0.0\% & 1292.2\% & -13.5\% & -86.7\% & {\cellcolor{green}} -96.4\% \\
% H2 cmplt P ccpvdz & 0.0\% & 1273.3\% & -17.5\% & -90.2\% & {\cellcolor{green}} -97.4\% \\
% LiH cmplt BK ccpvdz & 0.1\% & 1235.7\% & -11.8\% & -82.7\% & {\cellcolor{green}} -95.5\% \\
% H2 cmplt JW ccpvdz & 0.1\% & 1152.3\% & -24.6\% & -86.1\% & {\cellcolor{green}} -95.8\% \\
% H2O cmplt JW 631g & 0.1\% & 1149.9\% & -11.0\% & -81.6\% & {\cellcolor{green}} -96.4\% \\
% C2H4 frz JW sto3g & 0.1\% & 1347.1\% & -22.8\% & -86.1\% & {\cellcolor{green}} -95.1\% \\
% H2O cmplt P 631g & 0.1\% & 1156.1\% & -11.7\% & -82.7\% & {\cellcolor{green}} -96.9\% \\
% NH frz P sto3g & 0.2\% & 623.1\% & -49.9\% & -90.8\% & {\cellcolor{green}} -97.1\% \\
% H4 cmplt JW ccpvdz & 0.3\% & 1259.9\% & -33.8\% & -77.9\% & {\cellcolor{green}} -89.7\% \\
% LiH cmplt BK 631g & 0.3\% & 1194.3\% & -23.2\% & -79.1\% & {\cellcolor{green}} -91.0\% \\
% H4 cmplt BK ccpvdz & 0.3\% & 1228.8\% & -23.0\% & -80.1\% & {\cellcolor{green}} -89.5\% \\
% H2 cmplt JW 631g & 0.8\% & 1392.2\% & -27.9\% & -62.8\% & {\cellcolor{green}} -76.2\% \\
% LiH frz JW ccpvdz & 1.2\% & 704.6\% & -31.8\% & -70.6\% & {\cellcolor{green}} -86.5\% \\
% LiH cmplt BK sto3g & 1.3\% & 1010.5\% & -49.5\% & -78.6\% & {\cellcolor{green}} -87.4\% \\
% LiH frz BK sto3g & 0.9\% & 970.7\% & -27.5\% & -67.5\% & {\cellcolor{green}} -82.0\% \\
% NH frz P 631g & 0.8\% & 1202.2\% & -29.1\% & -64.7\% & {\cellcolor{green}} -76.3\% \\
% H8 cmplt JW sto3g & 0.8\% & 1269.9\% & -25.8\% & -64.1\% & {\cellcolor{green}} -75.3\% \\
% H2 cmplt P ccpvtz & 0.8\% & 1361.8\% & -18.5\% & -68.3\% & {\cellcolor{green}} -78.1\% \\
% C2H4 frz BK sto3g & 1.4\% & 1414.9\% & -12.8\% & -66.7\% & {\cellcolor{green}} -90.8\% \\
% H4 cmplt BK sto3g & 1.5\% & 1338.2\% & -18.6\% & -68.8\% & {\cellcolor{green}} -89.8\% \\
% H2 cmplt BK ccpvdz & 1.1\% & 1067.8\% & -28.5\% & -64.4\% & {\cellcolor{green}} -73.4\% \\
% \bottomrule
% \end{tabular}

%     \caption{Synthesis comparison for UCCSD Ansätze synthesis for different molecules, encodings, and bases. The first column displays the time taken by a naive python implementation. Other columns display the synthesis time relative to that value. The best result of each row is outlined in green.}
%     \label{tab:tab_chem_time_1}
% \end{table}

% \begin{table}[]
%     \centering

% \begin{tabular}{lrrrrr}
% \toprule
%  & naive & ph & tket & rdepth & rcount \\
%  & time & time & time & time & time \\
% name &  &  &  &  &  \\
% \midrule
% H2 cmplt P sto3g & 1.4\% & 1387.8\% & -41.1\% & -67.6\% & {\cellcolor{green}} -76.1\% \\
% H2O cmplt JW sto3g & 1.6\% & 2181.7\% & -5.4\% & -70.7\% & {\cellcolor{green}} -93.2\% \\
% LiH cmplt P ccpvdz & 1.6\% & 850.3\% & -47.6\% & -74.5\% & {\cellcolor{green}} -81.2\% \\
% LiH frz BK 631g & 1.5\% & 1396.9\% & -5.7\% & -68.1\% & {\cellcolor{green}} -91.9\% \\
% H2O frz BK sto3g & 1.6\% & 1359.9\% & -9.0\% & -70.0\% & {\cellcolor{green}} -92.4\% \\
% LiH frz JW sto3g & 1.5\% & 1118.6\% & -29.3\% & -59.2\% & {\cellcolor{green}} -66.8\% \\
% C2H4 cmplt P sto3g & 1.5\% & 1066.7\% & -23.3\% & -57.0\% & {\cellcolor{green}} -64.3\% \\
% LiH frz BK ccpvdz & 1.5\% & 1849.0\% & -29.2\% & -56.2\% & {\cellcolor{green}} -71.6\% \\
% LiH cmplt P 631g & 2.2\% & 1457.3\% & -28.5\% & -41.4\% & {\cellcolor{green}} -56.3\% \\
% H4 cmplt BK 631g & 2.3\% & 1287.3\% & -33.4\% & -52.5\% & {\cellcolor{green}} -53.6\% \\
% H8 cmplt BK sto3g & 2.1\% & 1237.3\% & -15.6\% & {\cellcolor{green}} -47.0\% & -42.1\% \\
% NH frz JW 631g & 2.6\% & 2053.3\% & -26.3\% & {\cellcolor{green}} -53.7\% & -48.9\% \\
% CH2 cmplt JW sto3g & 2.5\% & 1251.6\% & -25.9\% & -39.3\% & {\cellcolor{green}} -49.7\% \\
% CH2 cmplt BK sto3g & 5.3\% & 1610.0\% & {\cellcolor{green}} -32.1\% & -12.0\% & 2.9\% \\
% C2H4 frz P sto3g & 5.1\% & 1368.5\% & {\cellcolor{green}} -21.2\% & -13.4\% & 16.4\% \\
% H4 cmplt P sto3g & 5.8\% & 2283.4\% & {\cellcolor{green}} -38.7\% & -18.4\% & 1.9\% \\
% CH2 frz JW sto3g & 8.7\% & 2537.6\% & -9.9\% & -9.1\% & {\cellcolor{green}} -77.2\% \\
% H2 cmplt BK ccpvtz & 10.3\% & 6622.9\% & 19.7\% & 2.4\% & {\cellcolor{green}} -82.4\% \\
% H4 cmplt P ccpvdz & 11.8\% & 3489.7\% & -5.6\% & -15.8\% & {\cellcolor{green}} -84.2\% \\
% H2 cmplt BK sto3g & 8.1\% & 1638.8\% & -25.1\% & -14.6\% & {\cellcolor{green}} -56.3\% \\
% H2O cmplt BK sto3g & 9.6\% & 3430.5\% & -22.0\% & -11.7\% & {\cellcolor{green}} -50.9\% \\
% H4 cmplt JW sto3g & 11.4\% & 3137.7\% & {\cellcolor{green}} -27.6\% & 64.9\% & 115.3\% \\
% H2O cmplt BK 631g & 10.7\% & 1728.9\% & {\cellcolor{green}} -18.0\% & 52.1\% & 140.9\% \\
% NH cmplt BK 631g & 12.3\% & 1456.2\% & {\cellcolor{green}} -26.3\% & 73.4\% & 85.3\% \\
% \bottomrule
% \end{tabular}

% \caption{See table \ref{tab:tab_chem_time_1} for details}
%     \label{tab:tab_chem_time_2}
% \end{table}


% \begin{table}[]
%     \centering

% \begin{tabular}{lrrrrr}
% \toprule
%  & naive & ph & tket & rdepth & rcount \\
%  & time & time & time & time & time \\
% name &  &  &  &  &  \\
% \midrule
% H2O frz JW 631g & 48.2\% & 4623.7\% & -11.1\% & 112.3\% & {\cellcolor{green}} -75.3\% \\
% H2 cmplt BK 631g & 25.1\% & 2121.5\% & {\cellcolor{green}} -3.1\% & 166.2\% & 319.4\% \\
% NH cmplt JW 631g & 26.0\% & 3783.2\% & {\cellcolor{green}} -32.1\% & 149.8\% & 289.0\% \\
% LiH cmplt P sto3g & 31.8\% & 1583.5\% & {\cellcolor{green}} -32.6\% & 117.7\% & 196.5\% \\
% LiH frz P ccpvdz & 52.5\% & 12891.9\% & 34.6\% & 115.8\% & {\cellcolor{green}} -77.6\% \\
% CH2 frz BK sto3g & 57.6\% & 5865.6\% & 12.9\% & 79.7\% & {\cellcolor{green}} -78.3\% \\
% H4 cmplt JW 631g & 40.0\% & 2339.0\% & {\cellcolor{green}} -11.5\% & 251.9\% & 501.0\% \\
% LiH cmplt JW ccpvdz & 75.0\% & 2457.9\% & -22.9\% & 172.3\% & {\cellcolor{green}} -32.0\% \\
% C2H4 cmplt BK sto3g & 85.4\% & 2833.0\% & {\cellcolor{green}} -25.9\% & 256.7\% & 10.6\% \\
% H4 cmplt P 631g & 76.1\% & 7641.0\% & -5.2\% & 125.8\% & {\cellcolor{green}} -35.0\% \\
% H8 cmplt P sto3g & 80.2\% & 3539.3\% & -11.9\% & 111.7\% & {\cellcolor{green}} -29.0\% \\
% NH cmplt JW sto3g & 49.5\% & 2235.3\% & {\cellcolor{green}} -7.3\% & 339.5\% & 635.7\% \\
% NH frz BK sto3g & 51.7\% & 4742.8\% & {\cellcolor{green}} -22.8\% & 292.2\% & 654.1\% \\
% NH frz BK 631g & 52.6\% & 2180.4\% & {\cellcolor{green}} -29.1\% & 270.4\% & 604.7\% \\
% H2O frz P sto3g & 97.9\% & 7752.4\% & -1.8\% & 166.1\% & {\cellcolor{green}} -20.0\% \\
% NH frz JW sto3g & 93.4\% & 3924.5\% & -2.0\% & 142.0\% & {\cellcolor{green}} -18.4\% \\
% LiH frz JW 631g & 82.1\% & 2254.6\% & {\cellcolor{green}} -24.4\% & 382.2\% & 654.3\% \\
% NH cmplt P 631g & 82.3\% & 4707.7\% & {\cellcolor{green}} -27.4\% & 371.0\% & 655.6\% \\
% CH2 frz P sto3g & 69.7\% & 2630.2\% & {\cellcolor{green}} -5.4\% & 462.6\% & 775.8\% \\
% NH cmplt BK sto3g & 141.5\% & 2878.6\% & {\cellcolor{green}} -16.7\% & 650.3\% & 1136.8\% \\
% H2 cmplt JW ccpvtz & 148.9\% & 2094.1\% & {\cellcolor{green}} -9.5\% & 487.6\% & 1042.3\% \\
% H2 cmplt P 631g & 144.9\% & 4680.9\% & {\cellcolor{green}} -15.3\% & 511.8\% & 1038.9\% \\
% \bottomrule
% \end{tabular}

% \caption{See table \ref{tab:tab_chem_time_1} for details}
%     \label{tab:tab_chem_time_3}
% \end{table}


==> table_zx_counts.tex <==
\begin{tabular}{llrrrrrrrrrrrrr}
\toprule
 &  & init. & tket & par. & gs & ann. & ann.-r+gs & par.-r-ann. & gs-r-ann. & gs-r & g-c & g-c-ko & g-d & g-d-ko \\
nqbits & nops &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
\multirow[t]{6}{*}{10} & 1 & 3.8 & 7.6 & 3.8 & 3.8 & 3.9 & 3.8 & 8.6 & 8.8 & 3.8 & 3.8 & 3.8 & 3.8 & 3.8 \\
 & 2 & 11.9 & 16 & 7.7 & 8 & 9.2 & 7 & 16.4 & 15.6 & 8 & 6.9 & 6.9 & 8 & 8 \\
 & 5 & 35.9 & 32.2 & 15.9 & 16.8 & 21.4 & 14.1 & 30.4 & 30.9 & 16.8 & 15.4 & 15.5 & 18.2 & 18.1 \\
 & 10 & 81.7 & 60.8 & 28.7 & 34.3 & 53.3 & 29 & 56.3 & 55.8 & 34.3 & 29.9 & 30.7 & 35.6 & 35.7 \\
 & 50 & 415.3 & 295.2 & 99.2 & 134.4 & 332.1 & 121.7 & 151.7 & 155.4 & 134.4 & 128 & 126.2 & 147.7 & 142.3 \\
 & 100 & 845.3 & 584.5 & 171.5 & 234.6 & 701.2 & 214.6 & 253 & 251.9 & 234.6 & 217.2 & 215.1 & 257.1 & 254.2 \\
\cline{1-15}
\multirow[t]{6}{*}{15} & 1 & 7.2 & 14.4 & 7.2 & 7.2 & 7.8 & 7.2 & 15.8 & 15.6 & 7.2 & 7.2 & 7.2 & 7.2 & 7.2 \\
 & 2 & 18.5 & 21.2 & 11.4 & 11.9 & 13.5 & 10.7 & 23.5 & 22.8 & 11.9 & 10 & 10.2 & 12.3 & 12.3 \\
 & 5 & 60.5 & 52 & 24.9 & 29.2 & 39.2 & 24.8 & 53.4 & 53.6 & 29.2 & 23.2 & 23.7 & 30.7 & 31.1 \\
 & 10 & 129.2 & 97.6 & 48.4 & 56.1 & 90.4 & 48.5 & 102.2 & 103.4 & 56.1 & 49.1 & 49 & 62.8 & 64.4 \\
 & 50 & 654.2 & 448 & 189.2 & 241.5 & 539.4 & 222.9 & 295.4 & 296.1 & 241.5 & 234.8 & 236 & 273.7 & 287.3 \\
 & 100 & 1311.9 & 907.2 & 324.2 & 442 & 1147.6 & 421.1 & 500.4 & 504.1 & 442 & 447.7 & 448.6 & 526.6 & 538.7 \\
\cline{1-15}
\multirow[t]{6}{*}{20} & 1 & 9.6 & 19.2 & 9.6 & 9.6 & 10.2 & 9.6 & 20 & 20.2 & 9.6 & 9.6 & 9.6 & 9.6 & 9.6 \\
 & 2 & 28.2 & 33.4 & 15.6 & 15.9 & 21.2 & 14.9 & 33.4 & 31.4 & 15.9 & 14.5 & 14.5 & 16.8 & 16.8 \\
 & 5 & 80.6 & 71.4 & 38 & 41.6 & 57.6 & 36.6 & 77.4 & 78 & 41.6 & 33 & 32.9 & 44.3 & 44.2 \\
 & 10 & 172.3 & 134.5 & 67.4 & 74.3 & 124.8 & 65.7 & 141 & 140.3 & 74.3 & 67.3 & 66.2 & 82.3 & 85 \\
 & 50 & 888.9 & 630.8 & 270.3 & 364.5 & 769.6 & 336.5 & 467.5 & 463 & 364.5 & 369.4 & 380.6 & 431.6 & 442.3 \\
 & 100 & 1794.3 & 1198.3 & 497.7 & 691.6 & 1596.5 & 646.9 & 787.8 & 790 & 691.6 & 734.6 & 764.1 & 823.2 & 861 \\
\cline{1-15}
\multirow[t]{6}{*}{25} & 1 & 11.5 & 23 & 11.5 & 11.5 & 11.9 & 11.5 & 24.6 & 23.6 & 11.5 & 11.5 & 11.5 & 11.5 & 11.5 \\
 & 2 & 35.3 & 42.2 & 22.3 & 21.9 & 27.1 & 20.5 & 43.4 & 44.2 & 21.9 & 18.1 & 17.9 & 22.3 & 22.3 \\
 & 5 & 101 & 88.8 & 48.6 & 50.5 & 72.8 & 45.2 & 96.8 & 94.6 & 50.5 & 37.5 & 37.8 & 54.8 & 55.6 \\
 & 10 & 219.5 & 166 & 92 & 103.6 & 168.1 & 89.9 & 194.8 & 194.8 & 103.6 & 79.8 & 79.1 & 112.4 & 113.6 \\
 & 50 & 1155.2 & 772.4 & 387.6 & 479.8 & 999.9 & 457.1 & 652.8 & 654.7 & 479.8 & 530.7 & 550.5 & 571.9 & 593.4 \\
 & 100 & 2291.7 & 1556 & 699.1 & 914.8 & 2056.1 & 878.7 & 1086.4 & 1082.9 & 914.8 & 1095.7 & 1145.5 & 1124.3 & 1189.9 \\
\cline{1-15}
\bottomrule
\end{tabular}


==> table_zx_depths.tex <==
\begin{tabular}{llrrrrrrrrrrrrr}
\toprule
 &  & init. & tket & par. & gs & ann. & ann.-r+gs & par.-r-ann. & gs-r-ann. & gs-r & g-c & g-c-ko & g-d & g-d-ko \\
nqbits & nops &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
\multirow[t]{6}{*}{10} & 1 & 3.8 & 7.6 & 3.8 & 3.8 & 2.9 & 3.3 & 7.2 & 6.8 & 3.8 & 3.8 & 3.8 & 2.6 & 2.6 \\
 & 2 & 10.3 & 14.4 & 6.5 & 6.1 & 4.6 & 3.8 & 11.0 & 9.9 & 6.1 & 4.5 & 4.5 & 4.2 & 4.2 \\
 & 5 & 31.3 & 27.4 & 13.1 & 10.7 & 12.2 & 8.0 & 19.9 & 17.1 & 10.7 & 8.5 & 9.1 & 7.5 & 7.2 \\
 & 10 & 72.5 & 52.7 & 20.7 & 20.7 & 35.3 & 17.8 & 35.4 & 35.1 & 20.7 & 16.9 & 16.8 & 12.6 & 12.7 \\
 & 50 & 360.5 & 247.9 & 70.1 & 80.4 & 267.2 & 74.3 & 96.0 & 100.3 & 80.4 & 64.3 & 72.6 & 52.6 & 49.6 \\
 & 100 & 738.7 & 487.7 & 124.0 & 150.4 & 574.6 & 144.0 & 164.8 & 164.1 & 150.4 & 108.6 & 121.6 & 91.8 & 89.7 \\
\cline{1-15}
\multirow[t]{6}{*}{15} & 1 & 7.2 & 14.4 & 7.2 & 7.2 & 4.4 & 5.0 & 11.4 & 11.6 & 7.2 & 7.2 & 7.2 & 3.4 & 3.4 \\
 & 2 & 17.1 & 19.8 & 10.8 & 8.4 & 7.1 & 6.2 & 14.5 & 13.2 & 8.4 & 6.1 & 6.4 & 4.6 & 4.6 \\
 & 5 & 50.8 & 44.6 & 19.9 & 15.4 & 20.5 & 11.4 & 28.0 & 26.8 & 15.4 & 10.8 & 11.0 & 8.5 & 8.8 \\
 & 10 & 113.8 & 83.5 & 33.1 & 26.3 & 61.1 & 23.4 & 50.6 & 52.4 & 26.3 & 21.0 & 23.6 & 15.4 & 15.1 \\
 & 50 & 560.6 & 368.2 & 128.3 & 111.2 & 430.7 & 104.1 & 159.1 & 148.5 & 111.2 & 85.5 & 98.7 & 58.5 & 60.5 \\
 & 100 & 1130.4 & 751.9 & 213.1 & 205.1 & 947.6 & 199.2 & 250.0 & 256.2 & 205.1 & 162.6 & 191.7 & 113.0 & 113.8 \\
\cline{1-15}
\multirow[t]{6}{*}{20} & 1 & 9.6 & 19.2 & 9.6 & 9.6 & 5.3 & 7.3 & 16.0 & 16.6 & 9.6 & 9.6 & 9.6 & 3.8 & 3.8 \\
 & 2 & 26.2 & 31.4 & 13.0 & 10.8 & 10.1 & 8.8 & 20.4 & 19.8 & 10.8 & 8.6 & 8.7 & 5.2 & 5.2 \\
 & 5 & 71.3 & 62.8 & 29.2 & 18.6 & 33.7 & 15.9 & 36.8 & 31.8 & 18.6 & 11.9 & 12.9 & 9.6 & 9.7 \\
 & 10 & 152.1 & 115.5 & 50.2 & 30.2 & 86.0 & 24.6 & 57.6 & 56.6 & 30.2 & 22.1 & 25.5 & 14.9 & 15.4 \\
 & 50 & 773.0 & 526.1 & 182.2 & 127.7 & 633.3 & 121.3 & 213.4 & 206.4 & 127.7 & 110.9 & 127.1 & 66.2 & 67.5 \\
 & 100 & 1555.5 & 1000.4 & 338.5 & 243.4 & 1343.0 & 236.8 & 328.5 & 324.2 & 243.4 & 218.6 & 253.9 & 123.4 & 128.4 \\
\cline{1-15}
\multirow[t]{6}{*}{25} & 1 & 11.5 & 23.0 & 11.5 & 11.5 & 5.9 & 10.0 & 18.6 & 18.2 & 11.5 & 11.5 & 11.5 & 3.9 & 3.9 \\
 & 2 & 32.6 & 39.5 & 19.1 & 14.3 & 14.4 & 11.8 & 26.0 & 25.2 & 14.3 & 9.8 & 10.0 & 5.7 & 5.7 \\
 & 5 & 89.8 & 79.9 & 40.2 & 21.7 & 43.6 & 19.3 & 40.8 & 40.4 & 21.7 & 12.3 & 14.2 & 10.0 & 10.2 \\
 & 10 & 197.3 & 145.1 & 69.7 & 36.5 & 121.0 & 33.0 & 65.6 & 69.4 & 36.5 & 24.1 & 26.4 & 17.0 & 17.1 \\
 & 50 & 1006.4 & 650.7 & 281.1 & 137.3 & 832.1 & 131.9 & 270.7 & 271.2 & 137.3 & 140.8 & 155.9 & 69.0 & 69.1 \\
 & 100 & 1977.5 & 1298.9 & 479.5 & 263.5 & 1729.7 & 258.5 & 404.0 & 400.4 & 263.5 & 291.5 & 336.8 & 128.9 & 135.6 \\
\cline{1-15}
\bottomrule
\end{tabular}


==> table_zx_times.tex <==
\begin{tabular}{llrrrrrrrrrrrrr}
\toprule
 &  & init. & tket & par. & gs & ann. & ann.-r+gs & par.-r-ann. & gs-r-ann. & gs-r & g-c & g-c-ko & g-d & g-d-ko \\
nqbits & nops &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
\multirow[t]{6}{*}{10} & 1 & 0.0 & 0.2 & 0.0 & 0.0 & 0.0 & 2.0 & 0.2 & 0.3 & 0.6 & 0.0 & 0.0 & 0.0 & 0.0 \\
 & 2 & 0.0 & 0.3 & 0.0 & 0.0 & 0.0 & 2.8 & 0.4 & 0.4 & 1.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
 & 5 & 0.0 & 0.7 & 0.0 & 0.0 & 0.0 & 4.8 & 0.7 & 0.7 & 2.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
 & 10 & 0.0 & 1.3 & 0.1 & 0.0 & 0.1 & 6.6 & 0.9 & 0.9 & 2.7 & 0.0 & 0.0 & 0.0 & 0.0 \\
 & 50 & 0.1 & 6.0 & 0.3 & 0.1 & 0.2 & 11.7 & 1.8 & 1.8 & 6.4 & 0.0 & 0.0 & 0.0 & 0.0 \\
 & 100 & 0.2 & 12.2 & 0.5 & 0.1 & 0.3 & 17.8 & 2.9 & 2.9 & 11.3 & 0.0 & 0.0 & 0.0 & 0.0 \\
\cline{1-15}
\multirow[t]{6}{*}{15} & 1 & 0.0 & 0.3 & 0.1 & 0.0 & 0.0 & 5.5 & 0.7 & 0.7 & 1.6 & 0.0 & 0.0 & 0.0 & 0.0 \\
 & 2 & 0.0 & 0.5 & 0.1 & 0.0 & 0.0 & 7.3 & 1.0 & 1.0 & 2.6 & 0.0 & 0.0 & 0.0 & 0.0 \\
 & 5 & 0.0 & 1.1 & 0.2 & 0.1 & 0.1 & 18.1 & 2.4 & 2.5 & 6.7 & 0.0 & 0.0 & 0.0 & 0.0 \\
 & 10 & 0.1 & 2.1 & 0.4 & 0.1 & 0.1 & 23.0 & 3.2 & 3.3 & 9.6 & 0.0 & 0.0 & 0.0 & 0.0 \\
 & 50 & 0.3 & 9.7 & 1.1 & 0.2 & 0.4 & 37.2 & 5.6 & 5.7 & 19.7 & 0.0 & 0.0 & 0.0 & 0.0 \\
 & 100 & 0.7 & 20.2 & 1.9 & 0.4 & 0.9 & 54.7 & 8.7 & 8.7 & 32.7 & 0.1 & 0.1 & 0.0 & 0.0 \\
\cline{1-15}
\multirow[t]{6}{*}{20} & 1 & 0.0 & 0.5 & 0.3 & 0.0 & 0.0 & 11.9 & 1.5 & 1.5 & 3.3 & 0.0 & 0.0 & 0.0 & 0.0 \\
 & 2 & 0.0 & 0.8 & 0.3 & 0.1 & 0.0 & 15.6 & 2.3 & 2.2 & 5.1 & 0.0 & 0.0 & 0.0 & 0.0 \\
 & 5 & 0.1 & 1.6 & 0.8 & 0.2 & 0.1 & 47.5 & 6.3 & 6.4 & 17.8 & 0.0 & 0.0 & 0.0 & 0.0 \\
 & 10 & 0.2 & 3.0 & 1.2 & 0.3 & 0.2 & 64.8 & 9.0 & 9.1 & 25.3 & 0.0 & 0.0 & 0.0 & 0.0 \\
 & 50 & 0.9 & 14.6 & 3.7 & 0.5 & 1.0 & 94.8 & 14.1 & 14.0 & 46.1 & 0.1 & 0.1 & 0.0 & 0.0 \\
 & 100 & 1.7 & 29.0 & 6.3 & 0.8 & 2.1 & 130.9 & 20.5 & 20.5 & 76.0 & 0.2 & 0.3 & 0.1 & 0.1 \\
\cline{1-15}
\multirow[t]{6}{*}{25} & 1 & 0.0 & 0.6 & 0.6 & 0.1 & 0.0 & 21.2 & 2.7 & 2.5 & 5.9 & 0.0 & 0.0 & 0.0 & 0.0 \\
 & 2 & 0.1 & 1.0 & 1.2 & 0.1 & 0.1 & 36.6 & 4.6 & 5.1 & 11.4 & 0.0 & 0.0 & 0.0 & 0.0 \\
 & 5 & 0.2 & 2.2 & 2.1 & 0.5 & 0.1 & 99.7 & 13.4 & 13.7 & 34.5 & 0.0 & 0.0 & 0.0 & 0.0 \\
 & 10 & 0.4 & 4.0 & 3.6 & 0.7 & 0.3 & 152.4 & 20.3 & 20.4 & 51.7 & 0.0 & 0.0 & 0.0 & 0.0 \\
 & 50 & 2.0 & 19.0 & 11.4 & 1.2 & 2.0 & 216.6 & 31.5 & 31.6 & 101.5 & 0.2 & 0.2 & 0.0 & 0.0 \\
 & 100 & 3.9 & 39.7 & 18.1 & 1.6 & 4.1 & 275.4 & 42.0 & 42.1 & 147.4 & 0.5 & 0.6 & 0.1 & 0.1 \\
\cline{1-15}
\bottomrule
\end{tabular}

